Self-play Reinforcement Learning for Video Transmission

Video transmission services adopt adaptive algorithms to ensure users' demands. Existing techniques are often optimized and evaluated by a function that linearly combines several weighted metrics. Nevertheless, we observe that the given function fails to describe the requirement accurately. Thus, such proposed methods might eventually violate the original needs. To eliminate this concern, we propose \emph{Zwei}, a self-play reinforcement learning algorithm for video transmission tasks. Zwei aims to update the policy by straightforwardly utilizing the actual requirement. Technically, Zwei samples a number of trajectories from the same starting point and instantly estimates the win rate w.r.t the competition outcome. Here the competition result represents which trajectory is closer to the assigned requirement. Subsequently, Zwei optimizes the strategy by maximizing the win rate. To build Zwei, we develop simulation environments, design adequate neural network models, and invent training methods for dealing with different requirements on various video transmission scenarios. Trace-driven analysis over two representative tasks demonstrates that Zwei optimizes itself according to the assigned requirement faithfully, outperforming the state-of-the-art methods under all considered scenarios.

==> Zwei 4/abs.tex <==
\begin{abstract}
Video transmission services adopt adaptive algorithms to ensure users' demands.
Existing techniques are often optimized and evaluated by a function that linearly combines several weighted metrics.
Nevertheless, we observe that the given function fails to describe the requirement accurately. Thus, such proposed methods might eventually violate the original needs.
To eliminate this concern, we propose \emph{Zwei}, a self-play reinforcement learning algorithm for video transmission tasks. 
Zwei aims to update the policy by straightforwardly utilizing the actual requirement.
Technically, Zwei samples a number of trajectories from the same starting point, and instantly estimates the win rate w.r.t the competition outcome. 
Here the competition result represents which trajectory is closer to the assigned requirement. 
Subsequently, Zwei optimizes the strategy by maximizing the win rate.
To build Zwei, we develop simulation environments, design adequate neural network models, and invent training methods for dealing with different requirements on various video transmission scenarios. 
Trace-driven analysis over two representative tasks demonstrates that Zwei optimizes itself according to the assigned requirement faithfully, outperforming the state-of-the-art methods under all considered scenarios.
\end{abstract}


==> Zwei 4/conclusion.tex <==
\vspace{-10pt}
\section{Conclusion}
We propose Zwei, which utilize self-play RL to enhance itself based on the actual requirement, where the requirement is always hard to be described as a linear-based manner. We show that Zwei outperforms recent work with the improvements of more than 22\% on two representative video transmission tasks.
~(32.24\% on Elo score over the ABR scenario, 22\% on stalling ratio over the LTS).

\noindent \textbf{Acknowledgement.}~We thank the \emph{MMSys} and \emph{NOSSDAV} reviewer for the valuable feedback. This work was supported by NSFC under Grant 61936011, 61521002, Beijing Key Lab of Networked Multimedia, and National Key R\&D Program of China (No. 2018YFB1003703).

==> Zwei 4/details.tex <==
\begin{table*}[]
    \centering
    \caption{Details of ABR Tasks}
    \label{detail:1}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
        Trace Name & \multicolumn{2}{|c|}{BOLA} & \multicolumn{2}{|c|}{Rate-based} & \multicolumn{2}{|c|}{Pensieve} & \multicolumn{2}{|c|}{RobustMPC} & \multicolumn{2}{|c}{Zwei} \\ \hline
        - & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. \\ \hline
        bus 1 & 2659.6 & - & 2188.3 & - & 2480.9 & - & 2839.4 & 5.1 & \textbf{2802.1} & \textbf{-} \\ 
        bus 10 & 1467.0 & - & 1389.4 & 4.6 & 1413.8 & - & 1427.7 & 0.1 & \textbf{1490.4} & \textbf{-} \\ 
        bus 11 & 1327.7 & - & 1195.7 & - & 1264.9 & - & 1336.2 & 0.6 & \textbf{1363.8} & \textbf{-} \\ 
        bus 12 & 769.1 & 4.9 & 721.3 & - & 771.3 & 5.2 & 769.1 & 4.0 & \textbf{793.6} & \textbf{-} \\ 
        bus 13 & 852.1 & 9.7 & \textbf{529.8} & \textbf{-} & 623.4 & 2.6 & 629.8 & 5.5 & 666.0 & 0.7 \\ 
        bus 14 & 1675.5 & 8.3 & 933.0 & - & 1586.2 & 4.6 & 1610.6 & 4.6 & \textbf{1638.3} & \textbf{-} \\ 
        bus 15 & 3919.1 & - & 3497.9 & - & 3598.9 & - & \textbf{4141.5} & \textbf{-} & 3888.3 & - \\ 
        bus 16 & 3950.0 & - & 3652.1 & - & 3857.4 & - & \textbf{4145.7} & \textbf{-} & 3897.9 & - \\ 
        bus 17 & 1943.6 & - & 1844.7 & 2.2 & 1777.7 & - & 2005.3 & - & \textbf{2022.3} & \textbf{-} \\ 
        bus 18 & 1623.4 & - & 1559.6 & 0.4 & 1596.8 & - & 1588.3 & 1.0 & \textbf{1643.6} & \textbf{-} \\ 
        bus 19 & 1472.3 & - & 1212.8 & - & 1461.7 & - & 1440.4 & - & \textbf{1517.0} & \textbf{-} \\ 
        bus 2 & 1820.2 & - & 1656.4 & - & 1737.2 & - & 1861.7 & - & \textbf{1919.1} & \textbf{-} \\ 
        bus 20 & 1726.6 & - & 1517.0 & 1.6 & 1703.2 & - & 1752.1 & - & \textbf{1795.7} & \textbf{-} \\ 
        bus 21 & 1669.1 & - & 1497.9 & - & 1526.6 & - & 1759.6 & 2.1 & \textbf{1730.9} & \textbf{-} \\ 
        bus 22 & \textbf{1743.6} & \textbf{-} & 1594.7 & 7.8 & 1568.1 & - & 1791.5 & 3.6 & 1806.4 & 3.3 \\ 
        bus 23 & 1176.6 & 2.3 & 985.1 & 11.7 & 1076.6 & - & 1195.7 & 4.3 & \textbf{1178.7} & \textbf{-} \\ 
        bus 3 & 1331.9 & - & 1258.5 & - & 1283.0 & - & 1348.9 & 0.9 & \textbf{1368.1} & \textbf{-} \\ 
        bus 4 & 2121.3 & - & 1710.6 & - & 2103.2 & - & 2160.6 & 1.2 & \textbf{2156.4} & \textbf{-} \\ 
        bus 5 & 950.0 & 1.9 & 863.8 & 14.0 & 922.3 & - & \textbf{964.9} & \textbf{-} & 966.0 & - \\ 
        bus 6 & 1568.1 & - & 1324.5 & 0.3 & 1520.2 & - & 1606.4 & - & \textbf{1680.9} & \textbf{-} \\ 
        bus 7 & \textbf{2669.1} & \textbf{-} & 2376.6 & - & 2460.6 & - & 2571.3 & - & 2668.1 & - \\ 
        bus 8 & 2230.9 & - & 2008.5 & 2.9 & 2093.6 & - & \textbf{2305.3} & \textbf{-} & 2290.4 & - \\ 
        bus 9 & 2192.6 & - & 2014.9 & 4.0 & 2079.8 & - & 2297.9 & 1.8 & \textbf{2283.0} & \textbf{-} \\ 
        car 1 & 1440.4 & 0.8 & 1413.8 & 10.1 & 1467.0 & 12.7 & 1447.9 & 4.0 & \textbf{1434.0} & \textbf{-} \\ 
        car 10 & 1300.0 & - & 1127.7 & - & 1218.1 & - & 1338.3 & 2.6 & \textbf{1350.0} & \textbf{-} \\ 
        car 11 & 920.2 & 1.7 & 673.4 & 1.0 & 925.5 & - & 889.4 & - & \textbf{969.1} & \textbf{-} \\ 
        car 12 & 1291.5 & 18.2 & \textbf{1283.0} & \textbf{6.4} & 1291.5 & 13.7 & 1308.5 & 24.9 & 1325.5 & 13.5 \\ 
        car 2 & 1029.8 & - & 903.2 & - & 996.8 & - & 1034.0 & - & \textbf{1060.6} & \textbf{-} \\ 
        car 3 & 1351.1 & 1.8 & 1293.6 & - & 1334.0 & 2.0 & 1309.6 & 0.8 & \textbf{1327.7} & \textbf{-} \\ 
        car 4 & 1433.0 & 1.6 & 1327.7 & 3.4 & 1314.9 & - & 1423.4 & 1.7 & \textbf{1476.6} & \textbf{-} \\ 
        car 5 & 927.7 & 2.1 & 836.2 & 0.1 & 878.7 & - & 895.7 & - & \textbf{959.6} & \textbf{-} \\ 
        car 6 & 1295.7 & - & 1133.0 & - & 1263.8 & - & 1286.2 & - & \textbf{1326.6} & \textbf{-} \\ 
        car 7 & 710.6 & 1.3 & 568.1 & 11.9 & 666.0 & - & 677.7 & 0.9 & \textbf{697.9} & \textbf{-} \\ 
        car 8 & 1688.3 & - & 1448.9 & - & 1676.6 & - & 1704.3 & - & \textbf{1748.9} & \textbf{-} \\ 
        car 9 & 1485.1 & - & 1366.0 & - & 1423.4 & - & 1459.6 & - & \textbf{1526.6} & \textbf{-} \\ 
        ferry 1 & 1454.3 & 0.3 & 1423.4 & - & 1441.5 & - & 1455.3 & - & \textbf{1492.6} & \textbf{-} \\ 
        ferry 10 & 1119.1 & 0.2 & 1021.3 & 0.2 & 1104.3 & 0.2 & 1104.3 & 0.2 & \textbf{1133.0} & \textbf{0.2} \\ 
        ferry 11 & 1038.3 & 1.2 & 847.9 & - & 978.7 & - & 1037.2 & 0.1 & \textbf{1067.0} & \textbf{-} \\ 
        ferry 12 & 1525.5 & - & 1324.5 & 6.4 & 1466.0 & - & 1555.3 & - & \textbf{1586.2} & \textbf{-} \\ 
        ferry 13 & 1421.3 & 0.5 & 1192.6 & 12.6 & \textbf{1320.2} & \textbf{-} & 1436.2 & 5.4 & 1471.3 & 1.8 \\ 
        ferry 14 & 2036.2 & - & 1850.0 & 0.3 & 2074.5 & - & 2098.9 & - & \textbf{2124.5} & \textbf{-} \\ 
        ferry 15 & 1551.1 & - & 1385.1 & - & 1535.1 & - & 1486.2 & 1.1 & \textbf{1573.4} & \textbf{-} \\ 
        ferry 16 & 2684.0 & - & 2406.4 & - & 2480.9 & - & 2734.0 & - & \textbf{2817.0} & \textbf{-} \\ 
        ferry 17 & 859.6 & 0.1 & 768.1 & 9.4 & 818.1 & - & 826.6 & - & \textbf{850.0} & \textbf{-} \\ 
        ferry 18 & 724.5 & 2.8 & 587.2 & 4.9 & 666.0 & 1.1 & 667.0 & 1.0 & \textbf{684.0} & \textbf{-} \\ 
        ferry 19 & 839.4 & 4.8 & 654.3 & - & \textbf{826.6} & \textbf{-} & 825.5 & - & 863.8 & 7.1 \\ 
        ferry 2 & 1012.8 & 3.3 & 951.1 & 10.6 & 990.4 & - & 1001.1 & - & \textbf{1024.5} & \textbf{-} \\ \hline
    \end{tabular}
\end{table*}
\begin{table*}[]
    \centering
    \caption{Details of ABR Tasks}
    \label{detail:2}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
        Trace Name & \multicolumn{2}{|c|}{BOLA} & \multicolumn{2}{|c|}{Rate-based} & \multicolumn{2}{|c|}{Pensieve} & \multicolumn{2}{|c|}{RobustMPC} & \multicolumn{2}{|c}{Zwei} \\ \hline
        Trace Name & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. \\ \hline
        ferry 20 & 686.2 & 6.7 & 635.1 & - & 670.2 & 5.8 & 672.3 & 5.0 & \textbf{674.5} & \textbf{-} \\ 
        ferry 3 & 1211.7 & - & 1093.6 & - & 1170.2 & - & 1231.9 & 0.7 & \textbf{1252.1} & \textbf{-} \\ 
        ferry 4 & 562.8 & 4.2 & 472.3 & 1.9 & 543.6 & - & 558.5 & 4.7 & \textbf{563.8} & \textbf{-} \\ 
        ferry 5 & 1011.7 & 1.7 & 901.1 & 12.0 & 940.4 & - & 1018.1 & 2.2 & \textbf{1027.7} & \textbf{-} \\ 
        ferry 6 & 2014.9 & - & 1598.9 & - & 2039.4 & - & 2093.6 & - & \textbf{2119.1} & \textbf{-} \\ 
        ferry 7 & 1367.0 & 0.5 & 1231.9 & 1.4 & 1309.6 & - & 1346.8 & 0.6 & \textbf{1422.3} & \textbf{-} \\ 
        ferry 8 & 1078.7 & 3.8 & 1010.6 & - & 1076.6 & 1.7 & 1078.7 & 2.5 & \textbf{1105.3} & \textbf{-} \\ 
        ferry 9 & 964.9 & 3.8 & 787.2 & 5.1 & 868.1 & 3.7 & \textbf{898.9} & \textbf{1.9} & 1004.3 & 3.3 \\ 
        metro 1 & 1350.0 & - & 1141.5 & - & 1269.1 & - & 1371.3 & - & \textbf{1389.4} & \textbf{-} \\ 
        metro 10 & 896.8 & - & 625.5 & 3.7 & 837.2 & - & 895.7 & - & \textbf{935.1} & \textbf{-} \\ 
        metro 2 & 1364.9 & - & 1285.1 & 2.8 & 1316.0 & - & 1381.9 & 2.5 & \textbf{1409.6} & \textbf{-} \\ 
        metro 3 & 934.0 & - & 481.9 & - & 884.0 & - & 913.8 & - & \textbf{956.4} & \textbf{-} \\ 
        metro 4 & 1086.2 & 1.0 & 884.0 & 1.2 & 968.1 & 0.6 & 1030.9 & - & \textbf{1121.3} & \textbf{-} \\ 
        metro 5 & 1178.7 & 1.0 & 1041.5 & 3.8 & 1142.6 & - & \textbf{1171.3} & \textbf{-} & 1229.8 & 0.5 \\ 
        metro 6 & 577.7 & 0.9 & 386.2 & 6.6 & 558.5 & - & 548.9 & - & \textbf{573.4} & \textbf{-} \\ 
        metro 7 & 945.7 & - & 769.1 & - & 948.9 & 0.2 & 961.7 & 0.1 & \textbf{977.7} & \textbf{-} \\ 
        metro 8 & 740.4 & 2.5 & 443.6 & 6.4 & 738.3 & - & 724.5 & - & \textbf{762.8} & \textbf{-} \\ 
        metro 9 & 788.3 & - & 702.1 & 4.4 & 735.1 & - & 788.3 & 1.5 & \textbf{806.4} & \textbf{-} \\ 
        train 1 & 1028.7 & 4.2 & 863.8 & 2.3 & 996.8 & - & 1008.5 & - & \textbf{1024.5} & \textbf{-} \\ 
        train 10 & 1838.3 & - & 1627.7 & - & 1709.6 & - & 1894.7 & - & \textbf{1907.4} & \textbf{-} \\ 
        train 11 & 1256.4 & 0.4 & 1163.8 & 0.2 & 1171.3 & - & 1257.4 & - & \textbf{1286.2} & \textbf{-} \\ 
        train 12 & 1304.3 & 0.8 & 911.7 & 1.3 & 1114.9 & - & 1212.8 & - & \textbf{1380.9} & \textbf{-} \\ 
        train 13 & 1560.6 & - & 1236.2 & - & 1334.0 & - & 1564.9 & - & \textbf{1675.5} & \textbf{-} \\ 
        train 14 & 1330.9 & - & 1206.4 & - & 1259.6 & - & 1320.2 & - & \textbf{1356.4} & \textbf{-} \\ 
        train 15 & 1900.0 & - & 1423.4 & - & 1650.0 & - & \textbf{1952.1} & \textbf{-} & 1944.7 & - \\ 
        train 16 & 1661.7 & - & 1475.5 & 3.5 & 1484.0 & - & 1575.5 & - & \textbf{1736.2} & \textbf{-} \\ 
        train 17 & 1620.2 & - & 1394.7 & 4.1 & 1556.4 & - & 1637.2 & - & \textbf{1706.4} & \textbf{-} \\ 
        train 18 & 1978.7 & - & 1725.5 & - & 1803.2 & - & 2012.8 & - & \textbf{2091.5} & \textbf{-} \\ 
        train 19 & 1423.4 & - & 1230.9 & 2.5 & 1302.1 & - & 1452.1 & - & \textbf{1484.0} & \textbf{-} \\ 
        train 2 & 635.1 & 3.5 & 481.9 & 11.1 & \textbf{577.7} & \textbf{-} & 581.9 & - & 664.9 & 3.0 \\ 
        train 20 & 1331.9 & - & 1052.1 & - & 1343.6 & - & 1357.4 & - & \textbf{1373.4} & \textbf{-} \\ 
        train 21 & 1598.9 & - & 1421.3 & - & 1596.8 & - & 1626.6 & - & \textbf{1652.1} & \textbf{-} \\ 
        train 3 & 648.9 & 1.6 & 529.8 & 8.6 & 619.1 & - & 596.8 & - & \textbf{629.8} & \textbf{-} \\ 
        train 4 & 1084.0 & 3.3 & 868.1 & - & 1024.5 & - & 1059.6 & 0.3 & \textbf{1127.7} & \textbf{-} \\ 
        train 5 & 1241.5 & 1.5 & 946.8 & 0.4 & 1155.3 & - & 1151.1 & - & \textbf{1283.0} & \textbf{-} \\ 
        train 6 & 969.1 & 0.9 & 721.3 & - & 875.5 & - & 936.2 & 0.9 & \textbf{991.5} & \textbf{-} \\ 
        train 7 & 825.5 & 8.3 & 750.0 & - & \textbf{784.0} & \textbf{-} & 790.4 & - & 823.4 & 2.6 \\ 
        train 8 & 706.4 & 1.0 & 510.6 & - & 666.0 & - & 693.6 & - & \textbf{730.9} & \textbf{-} \\ 
        train 9 & 855.3 & - & 596.8 & - & 776.6 & - & 852.1 & - & \textbf{881.9} & \textbf{-} \\ 
        tram 1 & 635.1 & - & 472.3 & 1.6 & 625.5 & - & 635.1 & - & \textbf{656.4} & \textbf{-} \\ 
        tram 10 & 869.1 & 2.5 & 673.4 & - & 850.0 & - & \textbf{878.7} & \textbf{-} & 871.3 & - \\ 
        tram 11 & 587.2 & 4.3 & 472.3 & 1.3 & 558.5 & - & 548.9 & - & \textbf{580.9} & \textbf{-} \\ 
        tram 12 & 807.4 & - & 548.9 & - & 795.7 & - & 816.0 & - & \textbf{826.6} & \textbf{-} \\ 
        tram 13 & 788.3 & - & 596.8 & 0.9 & 739.4 & - & 787.2 & - & \textbf{831.9} & \textbf{-} \\ 
        tram 14 & 839.4 & 2.2 & 644.7 & 1.1 & 808.5 & - & 797.9 & - & \textbf{844.7} & \textbf{-} \\ 
        tram 15 & 453.2 & 6.9 & 357.4 & 5.3 & 414.9 & 1.8 & 424.5 & - & \textbf{437.2} & \textbf{-} \\ 
        tram 16 & \textbf{683.0} & \textbf{-} & 548.9 & - & 673.4 & - & 692.6 & - & 692.6 & - \\ 
        tram 17 & \textbf{654.3} & \textbf{-} & 424.5 & - & 625.5 & - & 635.1 & - & 663.8 & - \\ 
        tram 18 & 730.9 & 2.8 & 587.2 & - & 691.5 & - & 706.4 & - & \textbf{751.1} & \textbf{-} \\ \hline
    \end{tabular}
    %\caption{Details of ABR Tasks}
\end{table*}
\begin{table*}[]
    \centering
    \caption{Details of ABR Tasks}
    \label{detail:3}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
        Trace Name & \multicolumn{2}{|c|}{BOLA} & \multicolumn{2}{|c|}{Rate-based} & \multicolumn{2}{|c|}{Pensieve} & \multicolumn{2}{|c|}{RobustMPC} & \multicolumn{2}{|c}{Zwei} \\ \hline
        Trace Name & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. & Avg. Bit. & Rebuf. \\ \hline
        tram 19 & 967.0 & 0.1 & 788.3 & - & 907.4 & - & 973.4 & - & \textbf{985.1} & \textbf{-} \\ 
        tram 2 & 577.7 & 3.3 & 434.0 & - & 548.9 & - & 548.9 & - & \textbf{559.6} & \textbf{-} \\ 
        tram 20 & 930.9 & - & 730.9 & - & 885.1 & - & 928.7 & - & \textbf{988.3} & \textbf{-} \\ 
        tram 21 & 692.6 & 0.5 & 558.5 & - & 677.7 & - & 696.8 & - & \textbf{711.7} & \textbf{-} \\ 
        tram 22 & 510.6 & 0.3 & 376.6 & - & 491.5 & - & 501.1 & - & \textbf{506.4} & \textbf{-} \\ 
        tram 23 & 778.7 & - & 529.8 & - & 738.3 & - & 778.7 & - & \textbf{808.5} & \textbf{-} \\ 
        tram 24 & 788.3 & - & 616.0 & 3.4 & 739.4 & - & 769.1 & 0.3 & \textbf{808.5} & \textbf{-} \\ 
        tram 25 & 907.4 & - & 711.7 & - & 813.8 & - & 888.3 & - & \textbf{950.0} & \textbf{-} \\ 
        tram 26 & 568.1 & 0.8 & 300.0 & - & 539.4 & - & \textbf{568.1} & \textbf{-} & 567.0 & - \\ 
        tram 27 & \textbf{692.6} & \textbf{-} & 491.5 & - & 673.4 & - & 692.6 & - & 698.9 & - \\ 
        tram 28 & 558.5 & 0.3 & 386.2 & 2.2 & 510.6 & - & \textbf{539.4} & \textbf{-} & 540.4 & - \\  
        tram 29 & 510.6 & 3.4 & 338.3 & - & 481.9 & - & \textbf{501.1} & \textbf{-} & 495.7 & - \\ 
        tram 3 & 577.7 & 1.3 & 414.9 & - & \textbf{539.4} & \textbf{-} & 534.0 & 1.9 & 570.2 & 1.7 \\ 
        tram 30 & 692.6 & - & 319.1 & - & 644.7 & - & 687.2 & - & \textbf{719.1} & \textbf{-} \\ 
        tram 31 & 769.1 & - & 644.7 & - & 753.2 & - & 769.1 & - & \textbf{783.0} & \textbf{-} \\ 
        tram 32 & \textbf{788.3} & \textbf{-} & 558.5 & 1.7 & 733.0 & - & 750.0 & - & 788.3 & - \\ 
        tram 33 & \textbf{874.5} & \textbf{-} & 644.7 & - & 841.5 & - & 877.7 & 0.2 & 880.9 & - \\ 
        tram 34 & 926.6 & - & 778.7 & 1.6 & 917.0 & - & 930.9 & - & \textbf{959.6} & \textbf{-} \\ 
        tram 35 & 548.9 & 5.0 & 405.3 & 1.6 & 501.1 & - & 486.2 & - & \textbf{550.0} & \textbf{-} \\ 
        tram 36 & 850.0 & 0.3 & 539.4 & - & 819.1 & - & 816.0 & - & \textbf{874.5} & \textbf{-} \\ 
        tram 37 & 984.0 & - & 807.4 & - & 894.7 & - & 1003.2 & - & \textbf{1026.6} & \textbf{-} \\ 
        tram 38 & 644.7 & 9.6 & 481.9 & 4.5 & \textbf{591.5} & \textbf{-} & 625.5 & 4.9 & 646.8 & 2.3 \\ 
        tram 39 & 855.3 & - & 721.3 & - & 814.9 & - & 826.6 & - & \textbf{868.1} & \textbf{-} \\ 
        tram 4 & 462.8 & 5.2 & 300.0 & - & 414.9 & - & 414.9 & - & \textbf{428.7} & \textbf{-} \\ 
        tram 40 & 797.9 & 0.6 & 520.2 & 0.6 & 770.2 & 0.6 & 772.3 & 0.8 & \textbf{827.7} & \textbf{0.6} \\ 
        tram 41 & 769.1 & 2.8 & 663.8 & - & 734.0 & - & 750.0 & 0.5 & \textbf{785.1} & \textbf{-} \\ 
        tram 42 & 1069.1 & 9.0 & 692.6 & - & 961.7 & - & 1057.4 & - & \textbf{1076.6} & \textbf{-} \\ 
        tram 43 & 1079.8 & - & 960.6 & 0.2 & 1048.9 & - & 1084.0 & - & \textbf{1105.3} & \textbf{-} \\ 
        tram 44 & 869.1 & - & 759.6 & - & 801.1 & - & 874.5 & 0.7 & \textbf{893.6} & \textbf{-} \\ 
        tram 45 & 648.9 & 1.1 & 472.3 & 7.0 & \textbf{627.7} & \textbf{0.5} & 635.1 & 0.5 & 627.7 & 0.5 \\ 
        tram 46 & 683.0 & 4.2 & 414.9 & - & 606.4 & - & 662.8 & 0.1 & \textbf{679.8} & \textbf{-} \\ 
        tram 47 & 788.3 & 0.9 & 539.4 & - & 705.3 & - & 764.9 & - & \textbf{795.7} & \textbf{-} \\ 
        tram 48 & 616.0 & 0.3 & 395.7 & - & 558.5 & - & 605.3 & 0.2 & \textbf{619.1} & \textbf{-} \\ 
        tram 49 & 963.8 & 1.1 & 778.7 & - & 963.8 & - & 985.1 & 2.2 & \textbf{1007.4} & \textbf{-} \\ 
        tram 5 & 654.3 & 5.2 & 443.6 & 2.6 & 587.2 & - & 616.0 & - & \textbf{640.4} & \textbf{-} \\ 
        tram 50 & 863.8 & 6.8 & 797.9 & - & 851.1 & - & 845.7 & - & \textbf{864.9} & \textbf{-} \\ 
        tram 51 & 658.5 & 5.5 & 587.2 & - & \textbf{638.3} & \textbf{-} & 647.9 & - & 674.5 & 4.6 \\ 
        tram 52 & 920.2 & 3.4 & 788.3 & 1.7 & 905.3 & - & 903.2 & - & \textbf{927.7} & \textbf{-} \\ 
        tram 53 & 657.4 & 17.3 & 443.6 & 3.8 & 434.0 & 0.2 & 428.7 & - & \textbf{522.3} & \textbf{-} \\ 
        tram 54 & 1123.4 & 6.8 & 862.8 & 6.6 & 1059.6 & - & \textbf{1109.6} & \textbf{-} & 1106.4 & - \\ 
        tram 55 & 1176.6 & 0.4 & 1100.0 & - & 1141.5 & - & 1146.8 & 1.9 & \textbf{1177.7} & \textbf{-} \\ 
        tram 56 & 971.3 & - & 797.9 & - & 944.7 & - & 957.4 & - & \textbf{992.6} & \textbf{-} \\ 
        tram 6 & 740.4 & - & 587.2 & - & 683.0 & - & 744.7 & - & \textbf{784.0} & \textbf{-} \\ 
        tram 7 & 759.6 & - & 596.8 & - & 720.2 & - & 744.7 & - & \textbf{797.9} & \textbf{-} \\ 
        tram 8 & 501.1 & 3.5 & 414.9 & - & 472.3 & - & 462.8 & 0.2 & \textbf{483.0} & \textbf{-} \\ 
        tram 9 & 606.4 & 0.2 & 328.7 & - & 568.1 & - & 572.3 & - & \textbf{629.8} & \textbf{-} \\ \hline
    \end{tabular}
    %\caption{Details of ABR Tasks}
\end{table*}

==> Zwei 4/eval.tex <==

% \begin{table*}[]
%     \centering
%     \caption{We list the requirement and details for each video transmission task. Note that we label the underlying metric orderly since each metric has attentive priority. Hence, Zwei will learn the policy according to that sequence.}
%     \label{tbl:req}
%     \begin{tabular}{c|c|c|c|c}
%         \hline
%         Task Name & Transmission Type & Adaptive Bitrate & Requirement               & Constrain                \\ \hline
%         ABR~(\S\ref{sec:abr})       & \emph{\textbf{Client-to-Server}}  & \checkmark              & \down{Rebuffering Time$^1$}, \up{Bitrate$2$} & Bitrate $\Leftrightarrow$ Rebuffering Time \\
%         CLS~(\S\ref{sec:cls})       & \emph{\textbf{Server-to-Client}}  & $\times$               & \down{Stalling Ratio$^1$}, \down{Cost$^2$}         & Stalling Ratio $\Leftrightarrow$ Cost        \\
%         RTC~(\S\ref{sec:rtc})       & \emph{\textbf{Client-to-Client}}  & \checkmark              & \down{RTT$^1$}, \down{Loss$^1$}, \up{Bitrate$^2$}        & Bitrate $\Leftrightarrow$ (RTT\&Loss)     \\ \hline
%     \end{tabular}
% \end{table*}


\section{Evaluation}
\label{sec:eval}
In this section, we thoroughly evaluate the performance of Zwei over two representative scenarios.

\subsection{Zwei's NN Implementation}
We use TensorFlow~\cite{abadi2016tensorflow} to construct Zwei. 
%Zwei consists of two NNs, policy network and outcome network. 
Zwei's policy network takes a n-dims vector with \emph{softmax} active function as the output, and the outcome network outputs a value with \emph{tanh} function scaled in $(-1, 1)$.
Considering the characteristics on video transmission tasks, we construct different NN architectures for each task, but use the same set of hyper-parameters for training the NN: sample number $N=16$, learning rate $\alpha=10^{-4}$. 
% In addition, we adopt Adam optimizer~\cite{kingma2014adam} with default settings. 
Notice that we discuss the NN architecture and the effect of different sample number in \S\ref{sec:abr}.

% More details, including \textbf{NN architecture details, hyperparameters, and additional experiments} are demonstrated in the \textbf{\emph{supplementary materials}}.
\subsection{ABR Scenarios}
\label{sec:abr}
% We first understand how Zwei works in the ABR scenario.
% Detailing the working process, that includes, testbed setup, baseline introduction, and Zwei vs. Existing ABR schemes.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figs/outabr0}
%     \caption{This figure shows the typical ABR System.}
%     \label{fig:abr0}
% \end{figure}

\subsubsection{ABR's Background}
% Due to the rapid development of network services, watching video streaming online has become an upcoming trend. Today, adaptive video streaming, such as HLS~(HTTP Live Streaming)~\cite{HLS} and DASH~\cite{dash}, an algorithm that dynamically selects video bitrates via network conditions and client's buffer occupancy, is the predominant form of video delivery~\cite{bentaleb2018survey}. 
The ABR video streaming architecture consists of a video player client with a constrained buffer length and an HTTP-Server or Content Delivery Network~(CDN). The video player client decodes and renders video frames from the playback buffer. Once the streaming service starts, the client fetches the video chunk from the HTTP Server or CDN orderly by an ABR algorithm. The algorithm determines next chunks' video quality.
After finished to play the video, several metrics, such as total bitrate, total re-buffering time and total bitrate change will be summarized as a QoE metric to evaluate the performance.
% Thus, achieving a high QoE score for video streaming has become a major challenge for ABR algorithms. 


% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\linewidth]{figs/bitrate}
%     \includegraphics[width=0.4\linewidth]{figs/bufrat}
%     % \begin{minipage}{0.48\linewidth}
%     %     \centering
%     %     \subfigure{\includegraphics[width=1.0\textwidth]{figs/motivation/vmaf-phone-score}}
%     % \end{minipage}     
%     % \begin{minipage}{0.24\linewidth}
%     %     \centering
%     %     \subfigure{\includegraphics[width=1.0\textwidth]{figs/motivation/vmaf-score-fit3}}
%     % \end{minipage}
%     \caption{Comparing the strategy between the virtual player and real \texttt{Dash.js} player. Results show the close correlation of strategy between the two players.}
%     \label{fig:virtualplayer}
%     %\vspace{-10pt}
% \end{figure}

% \subsubsection{Virtual Player Evaluation}
% We design a faithful ABR offline virtual player to train Zwei with the given network traces and video descriptions. The player is written in Python3.6 and is closely refers to several state-of-the-art open-sourced ABR simulators including Pensieve, Oboe and Sabre~\cite{spiteri2018theory}. Besides, We verify the accurateness of the proposed virtual player in Figure~\ref{fig:virtualplayer}.

\begin{figure*}
    \centering
    % \subfigure[Typical ABR System.]{
    %     \includegraphics[width=0.23\linewidth]{figs/outabr0}}
    \subfigure[Zwei vs. ABR schemes]{
        \includegraphics[width=0.23\linewidth]{figs/elo-fc}
        \label{fig:abr:a}}
    \subfigure[Zwei vs. Tiyuntsong]{
        \includegraphics[width=0.23\linewidth]{figs/elo3}
        \label{fig:abr:b}}
    \subfigure[ABR Scheme Details]{
    \includegraphics[width=0.23\linewidth]{figs/out}
        \label{fig:abr:c}}
    \subfigure[CDF of ABR Algorithms]{
    \includegraphics[width=0.23\linewidth]{figs/cdf-4-3}
        \label{fig:abr:d}}
    \vspace{-15pt}  
    \caption{This group of figures show the comparison results of Zwei and other ABR approaches. Results are evaluated in the typical ABR system with HD Videos~(video resolution=1920 $\times$ 1080, maximum bitrate=4.3mbps).}
    \label{fig:abr}
\end{figure*}

\subsubsection{NN Architecture}
We now explain the details of the Zwei's neural network~(NN), including its inputs, outputs, network architecture, and implementation.

\textbf{Inputs.}
For each chunk $k=8$, Zwei takes the state inputs $S_k=\{X_k, \tau_k, N_k, b_k, c_k, l_k\}$ as the input, in which $X_k$ represents the throughput measured for past $t$ times, $\tau_k$ reflects the vector of download time for past $t$ chunks, $N_k$ is the next video sizes for each bitrate chunk, $b_k$ means current buffer occupancy, $l_k$ is the normalized value of the last bitrate selected, $c_k$ is the scalar which means the video chunk remaining. 

\textbf{Outputs.}
We attempt to use discrete action space to describe the output. Note that the output is an n-dim vector indicating the probability of the bitrate being selected under the current ABR state $S_k$. In this work, we set $n=6$, which is widely used in ABR papers~\cite{huang2018tiyuntsong,mao2017neural}.



\textbf{NN Representation.}
Zwei's NN representation is quite simple: it leverages three fully-connected layers, which is sized 128, 64, and 64 respectively, for describing the feature extraction layer. The output of the NN's policy network is a \emph{6-dims} vector, which represents the probabilities for each bitrate selected. The NN's outcome network outputs a value scaled in (-1, 1).


\textbf{Requirements for ABR tasks.}
Algorithm~\ref{alg:Overall} is an example of Rule $\texttt{Rule}$ which used in the ABR scenario, where $\epsilon_{c}$ is a small number that can add noise for improving Zwei's robustness. In this work, we set $\epsilon_{c}$ as 10. Note that, such settings are trivial and you can just set the value as a small value~(e.g., 0.1) instead.

\begin{small}
\begin{algorithm}
\caption{Rule for the ABR task.} 
\label{alg:Overall} 
\begin{algorithmic}[1]
\Require Trajectory $T_{u}, T_{v}$;
\State Compute average bitrate $r_{u}, r_{v}$, average rebuffering $b_{u}, b_{v}$ from the given trajectories $T_{u}, T_{v}$. \Comment Requirements: i) low rebuffering time ii) high bitrate.
\State Initialize Return $s=\{-1, -1\}$;
\If{$\left| b_{u} - b_{v} \right|< \epsilon_{c}$ or $\left| r_{u} - r_{v} \right|< \epsilon_{c}$}
\State Randomly set $s_{0}$ or $s_{1}$ as 1. 
\Comment Add noise to improve the robustness.
\ElsIf{$\left| b_{u} - b_{v} \right|<\epsilon_{c}$}
\State $s_i \gets 1, i={argmax}_{i\in \{u,v\}}{r}$;
\Else
\State $s_i \gets 1, i={argmin}_{i\in \{u,v\}}{b}$;
\EndIf
\State return $s$;
%\EndProcedure
\end{algorithmic} 
\end{algorithm}
\end{small}

\textbf{QoE Representation.}
Recall that the goal of ABR algorithm is to select bitrates for the next chunk $k$ with high bitrate $r_k$ and less rebuffering time $t_k$~\cite{mao2019real}, thus the optimization reward $q_k$ can be normally written as $q_k = r_k - \alpha t_k$, here $\alpha$ is the coefficient that adjust the importance of the underlying metrics. Note that prior research often add additional smoothness metric $\left| r_k - r_{k-1} \right|$ to control the bitrate change of the entire session, while in practice the following metric is neglectable for the ABR algorithm~\cite{mao2019real,Huang2019Hindsight}. Hence, in this work we also set the smoothness to zero for better understanding the fundamental performance of Zwei. Solving Zwei with smoothness metric will be our future work.

\begin{figure*}
    \centering
    \subfigure[Zwei vs. ABR schemes]{
        \includegraphics[width=0.23\linewidth]{figs/elo-12}
        \label{fig:abr2:a}}
    \subfigure[Zwei with Different Samples]{
        \includegraphics[width=0.23\linewidth]{figs/elo2}
        \label{fig:abr2:b}}
    \subfigure[ABR Algorithm Details]{
    \includegraphics[width=0.23\linewidth]{figs/out12}
    \label{fig:abr2:c}}
    \subfigure[CDF of ABR Algorithms]{
    \includegraphics[width=0.23\linewidth]{figs/cdf-12}
    \label{fig:abr2:d}}
    \vspace{-15pt}
    \caption{This group of figures show the comparison results of Zwei and other ABR approaches. Results are evaluated in the typical ABR system with 4K Videos~(video resolution=3840 $\times$ 2160, maximum bitrate=12.0mbps).}
    %\vspace{-10pt}
    \label{fig:abr2}
\end{figure*}


\subsubsection{Experimental Setup} We employ the standard ABR's emulation environment~\cite{mao2017neural} to evaluate Zwei. We adopt various network bandwidth databases, including HSDPA~\cite{riiser2013commute}, FCC~\cite{bworld}. Training process lasts approximate 45000 steps, within 10 hours to obtain a reliable result. In this experiment, we setup two ABR scenarios, i.e., HD and 4K video scenario. In the HD video scenario, we adopt \emph{EnvivioDash3}, a video that commonly used in recent work~\cite{mao2017neural}, to validate Zwei, where the video chunks are encoded as $\{0.3, 0.75, 1.2, 1.8, 2.8, 4.3\}$ mbps. In the 4K-video scenario, we use the popular open-source movie Big Buck Bunny~\cite{bbb2020}, which is now even more a world standard for video standards. Specifically, we pick 6 bitrates from \texttt{Dash.js} standard~\cite{dash}, i.e., $\{0.2, 0.6, 1.5, 4.0, 8.0, 12.0\}$ mbps.
% ~\footnote{We deleted some unnecessary bitrates that RL-based scheme seldom picks, e.g., $\{1.2, 2.85\}$ mbps~\cite{dethise2019cracking}.}

\textbf{ABR Baselines.}
In this paper, we select several representational ABR algorithms from various type of fundamental principles:
\begin{enumerate}[leftmargin=*]
    \label{sec:abrbaseline}
    \item \textbf{\emph{Rate-based}~\cite{jiang2014improving}:}~the basic baseline for ABR problems. It leverages \emph{harmonic mean} of past five throughput measured as future bandwidth.
    
    \item \textbf{\emph{BOLA}~\cite{spiteri2016bola}:}~the most popular buffer-based ABR scheme in practice. BOLA turns the ABR problem into a utility maximization problem and solve it by using the Lyapunov function.
    
    \item \textbf{\emph{RobustMPC}~\cite{yin2015control}:}~a state-of-the-art heuristic method which maximizes the objectives by jointly considered the buffer occupancy and throughput predictions. We implement \emph{RobustMPC} by ourselves.

    \item \textbf{\emph{Pensieve}~\cite{mao2017neural}:}~the state-of-the-art learning-based ABR scheme which utilizes DRL to select bitrate for next video chunks.
    
    \item \textbf{\emph{Tiyuntsong}~\cite{huang2018tiyuntsong}:}~the first study of multi-objective optimization ABR approach. Tiyuntsong uses actor-critic method to update the NN via the competition with two agents under the same network condition. 
\end{enumerate}

\textbf{Evaluation Metrics} The Elo rating~\cite{coulom2008whole} is a traditional method for calculating the relative performance of players in zero-sum games. It's suitable to compare different schemes via win rate information only. Thus, we also use Elo score to compare different ABR schemes, similar to that of AlphaGo~\cite{silver2016mastering} and Tiyuntsong~\cite{huang2018tiyuntsong}.

% \begin{figure}
%     \centering
%         \includegraphics[width=0.48\linewidth]{figs/cdf-bitrate}
%         \includegraphics[width=0.48\linewidth]{figs/cdf-rebuf}
%         %\vspace{-10pt}
%     \caption{Here is the CDF distribution of average bitrate and rebuffering time for the selected approaches.}
%     %\vspace{-10pt}
%     \label{fig:abr2}
% \end{figure}


\subsubsection{HD Video} We study the performance of Zwei over the HD video dataset and HSDPA network traces. Followed by recent work~\cite{yin2015control}, we set $\alpha$ = 4.3 as the basic QoE-HD metric.

\textbf{Zwei vs. Existing schemes.}~
In this experiment, we compare Zwei with existing ABR schemes over the HSDPA dataset. Results are computed as the Elo-score and reported in Figure~\ref{fig:abr:a}. Specifically, we first select several previously proposed approaches and validate the performance respectively under the \emph{same} network and video environment. Next, we use \texttt{Rule} to estimate their winning rate. Finally, we compute the Elo rating for these approaches.

Through the experiments we can see that Zwei outperforms recent ABR approaches. In particular, Zwei improves Elo-score on 36.38\% compared with state-of-the-art learning-based method Pensieve, and increases 31.11\% in terms of state-of-the-art heuristic method RobustMPC. Same conclusion are demonstrated as the CDF of QoE in Figure~\ref{fig:abr:d}.
Besides, we also illustrate the comparison results of different methods on average bitrate and average rebuffering in Figure~\ref{fig:abr:c}. As shown, Zwei can not only achieve highest bitrate but also obtain lowest rebuffering under all network traces. 
We compare Zwei with previously proposed self-learning method Tiyuntsong on the same experimental setting. Results are shown as the Elo-curve in Figure~\ref{fig:abr:b}. As expected, Zwei with any NN architectures outperforms Tiyuntsong on average Elo-score of 35\%.
The reason is that Tiyuntsong treat the learning process as a battle with two separated NNs, as each agent have to use the sample only collected by the agent itself. Thus, it lacks sample efficiency and sometimes struggles into the sub-optimal solution. 
% On the contrary, Zwei leverages more than \emph{belligerents} for sampling, aiming to update one NN together. Because each agent will share its experience with the others, Zwei can achieve sample efficiency.
% compared with Tiyuntsong.
% Moreover, Tiyuntsong is also a self-play learning method which uses conventional actor-critic method to update the NN for obtaining a higher $Q_t$, where $Q_t$ is cumulative reward $Q_t = r_t + \gamma Q_{t+1} $, where $\gamma=0.99$. Tiyuntsong is the special case of Zwei.

\textbf{Zwei with Different NN Architectures.}
This experiment considers Zwei with several NN architectures, where Zwei-1D is the standard ABR NN architecture~\cite{mao2017neural}, Zwei-2D uses stacked Conv-2D layers to extract features, and Zwei takes three fully-connected layers sized $\{128, 64, 64\}$. Results are shown in Figure~\ref{fig:abr:b}.  Unsurprisingly, when Zwei trains with some complicated NN architecture~(i.e., Zwei-1D and Zwei-2D), it performs worse than the fully connected NN scheme. This makes sense since ABR is a light-weighted task which can be solved in a practical and uncomplicated manner instead of a NN incorporating some \emph{deep} yet \emph{wide} layers.

% \textbf{The Two-Stage Phenomenon.}
% By meticulously observing Zwei's training curve on Figure~\ref{fig:abr}(a), we find the training process can be split into two stages: 1)~Zwei picked a lower bitrate to avoid rebuffering time when the training step is less than 100. Then 2)~Zwei realized a new strategy and increased the bitrate with guaranteeing rebuffering events. The reason is Zwei skillfully exploits catastrophic forgetting~\cite{goodfellow2013empirical} and abandons far-reaching decisions.

% \begin{figure*}
%     \centering
%     \subfigure[Zwei vs. ABR schemes]{
%         \includegraphics[width=0.23\linewidth]{figs/Elo-12}}
%     \subfigure[Zwei vs. Tiyuntsong]{
%         \includegraphics[width=0.23\linewidth]{figs/Elo2}}
%     \subfigure[ABR Scheme Details]{
%     \includegraphics[width=0.23\linewidth]{figs/cdf-12}}
%         %\vspace{-10pt}
%     \caption{Here is the CDF distribution of average bitrate and rebuffering time for the selected approaches.}
%     %\vspace{-10pt}
%     \label{fig:abr2}
% \end{figure*}

\subsubsection{4K Video} we evaluate Zwei with 4K videos on HDFS network traces, and the video are encoded with $\{0.2, 0.6, 1.5, 4.0, 8.0, 12.0\}$ mbps.
In particular, we have also retrained Pensieve with the Big Buck Bunny and QoE-4K. 
%Results illustrate that Pensieve outperforms RobustMPC, with an overall average QoE improvements of 2.67\% across all sessions. 

\textbf{QoE metrics for other approaches.} Due to the difference between the maximum bitrate of 4K video~(i.e., 12mbps) and HD video~(i.e., 4.3mbps), we refer $QoE_4K$ as the QoE function for other ABRs~(expect Zwei). Specifically, we set the penalty of rebuffering parameter $\alpha$ to 20 for better avoiding the occurrence of rebuffering.

\textbf{Zwei vs. Recent ABR Schemes.} Figure~\ref{fig:abr2:a} plots the learning curves in terms of the comparison of Zwei and other ABR methods. We observe that Zwei has already achieved state-of-the-art performance in almost 200 epochs, and finally,  the performance improvement of Zwei can achieve 32.24\% against the second best algorithm Pensieve and 58.58\%-120.76\% against others. What's more, as depicted in Figure~\ref{fig:abr2:c}, no matter average bitrate or total rebuffering time, Zwei always stands for the best scheme among all candidates. In particular, Zwei increases 10.46\% on average bitrates with reducing 56.52\% on total rebuffering time. Meanwhile, we also report the comparison of QoE performance of the proposed scheme in Figure~\ref{fig:abr2:d}. As expected, Zwei outperforms existing ABR algorithms without reward engineering, with the increasing on average QoE of 11.59\%.

\textbf{Zwei with Different Samples $N$.}~Besides, we also investigate the Elo-rating of Zwei with different sample $N$, where we set $N=\{2,4,8,16\}$. Figure~\ref{fig:abr2:b} illustrates the comparison of each method, we observe that Zwei can achieve sample efficiency with the increasing of the sample number $N$.
% \begin{table*}[]
%     \centering
%     \caption{Details of ABR Tasks}
%     \label{detail:1}
%     %\begin{small}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%     \hline
%         Trace ID & \multicolumn{2}{|c|}{BOLA} & \multicolumn{2}{|c|}{Rate-based} & \multicolumn{2}{|c|}{Pensieve} & \multicolumn{2}{|c|}{RobustMPC} & \multicolumn{2}{|c}{Zwei} \\ \hline
%         - & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Bitrate\\ (KBps)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total \\ Rebuffering\\ (s)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Bitrate\\ (KBps)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total \\ Rebuffering\\ (s)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Bitrate\\ (KBps)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total \\ Rebuffering\\ (s)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Bitrate\\ (KBps)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total \\ Rebuffering\\ (s)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Avg. \\ Bitrate\\ (KBps)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Total \\ Rebuffering\\ (s)\end{tabular}} \\ \hline
%         1 & 2659.6 & - & 2188.3 & - & 2480.9 & - & 2839.4 & 5.1 & \textbf{2802.1} & \textbf{-} \\ 
%         2 & 1467.0 & - & 1389.4 & 4.6 & 1413.8 & - & 1427.7 & 0.1 & \textbf{1490.4} & \textbf{-} \\ 
%         3 & 1327.7 & - & 1195.7 & - & 1264.9 & - & 1336.2 & 0.6 & \textbf{1363.8} & \textbf{-} \\ 
%         4 & 769.1 & 4.9 & 721.3 & - & 771.3 & 5.2 & 769.1 & 4.0 & \textbf{793.6} & \textbf{-} \\ 
%         5 & 852.1 & 9.7 & \textbf{529.8} & \textbf{-} & 623.4 & 2.6 & 629.8 & 5.5 & 666.0 & 0.7 \\ 
%         6 & 1675.5 & 8.3 & 933.0 & - & 1586.2 & 4.6 & 1610.6 & 4.6 & \textbf{1638.3} & \textbf{-} \\ 
%         7 & 3919.1 & - & 3497.9 & - & 3598.9 & - & \textbf{4141.5} & \textbf{-} & 3888.3 & - \\ 
%         8 & 1029.8 & - & 903.2 & - & 996.8 & - & 1034.0 & - & \textbf{1060.6} & \textbf{-} \\ 
%         9 & 1943.6 & - & 1844.7 & 2.2 & 1777.7 & - & 2005.3 & - & \textbf{2022.3} & \textbf{-} \\ 
%         10 & 1623.4 & - & 1559.6 & 0.4 & 1596.8 & - & 1588.3 & 1.0 & \textbf{1643.6} & \textbf{-} \\ 
%         11 & 1472.3 & - & 1212.8 & - & 1461.7 & - & 1440.4 & - & \textbf{1517.0} & \textbf{-} \\ 
%         12 & 1820.2 & - & 1656.4 & - & 1737.2 & - & 1861.7 & - & \textbf{1919.1} & \textbf{-} \\ 
%         13 & 1726.6 & - & 1517.0 & 1.6 & 1703.2 & - & 1752.1 & - & \textbf{1795.7} & \textbf{-} \\ 
%         14 & 1669.1 & - & 1497.9 & - & 1526.6 & - & 1759.6 & 2.1 & \textbf{1730.9} & \textbf{-} \\ 
%         15 & \textbf{1743.6} & \textbf{-} & 1594.7 & 7.8 & 1568.1 & - & 1791.5 & 3.6 & 1806.4 & 3.3 \\ 
%         16 & 1176.6 & 2.3 & 985.1 & 11.7 & 1076.6 & - & 1195.7 & 4.3 & \textbf{1178.7} & \textbf{-} \\ 
%         17 & 1331.9 & - & 1258.5 & - & 1283.0 & - & 1348.9 & 0.9 & \textbf{1368.1} & \textbf{-} \\ 
%         18 & 2121.3 & - & 1710.6 & - & 2103.2 & - & 2160.6 & 1.2 & \textbf{2156.4} & \textbf{-} \\ 
%         19 & 950.0 & 1.9 & 863.8 & 14.0 & 922.3 & - & 964.9 & - & \textbf{966.0} & \textbf{-} \\ 
%         20 & 1568.1 & - & 1324.5 & 0.3 & 1520.2 & - & 1606.4 & - & \textbf{1680.9} & \textbf{-} \\ 
%         21 & \textbf{2669.1} & \textbf{-} & 2376.6 & - & 2460.6 & - & 2571.3 & - & 2668.1 & - \\ 
%         22 & 2192.6 & - & 2014.9 & 4.0 & 2079.8 & - & 2297.9 & 1.8 & \textbf{2283.0} & \textbf{-} \\ 
%         23 & 1440.4 & 0.8 & 1413.8 & 10.1 & 1467.0 & 12.7 & 1447.9 & 4.0 & \textbf{1434.0} & \textbf{-} \\ 
%         24 & 1300.0 & - & 1127.7 & - & 1218.1 & - & 1338.3 & 2.6 & \textbf{1350.0} & \textbf{-} \\ 
%         25 & 920.2 & 1.7 & 673.4 & 1.0 & 925.5 & - & 889.4 & - & \textbf{969.1} & \textbf{-} \\ 
%         % car 12 & 1291.5 & 18.2 & \textbf{1283.0} & \textbf{6.4} & 1291.5 & 13.7 & 1308.5 & 24.9 & 1325.5 & 13.5 \\ 
%         % car 2 & 1029.8 & - & 903.2 & - & 996.8 & - & 1034.0 & - & \textbf{1060.6} & \textbf{-} \\ 
%         % car 3 & 1351.1 & 1.8 & 1293.6 & - & 1334.0 & 2.0 & 1309.6 & 0.8 & \textbf{1327.7} & \textbf{-} \\ 
%         % car 4 & 1433.0 & 1.6 & 1327.7 & 3.4 & 1314.9 & - & 1423.4 & 1.7 & \textbf{1476.6} & \textbf{-} \\ 
%         % car 5 & 927.7 & 2.1 & 836.2 & 0.1 & 878.7 & - & 895.7 & - & \textbf{959.6} & \textbf{-} \\ 
%         % car 6 & 1295.7 & - & 1133.0 & - & 1263.8 & - & 1286.2 & - & \textbf{1326.6} & \textbf{-} \\ 
%         % car 7 & 710.6 & 1.3 & 568.1 & 11.9 & 666.0 & - & 677.7 & 0.9 & \textbf{697.9} & \textbf{-} \\ 
%         % car 8 & 1688.3 & - & 1448.9 & - & 1676.6 & - & 1704.3 & - & \textbf{1748.9} & \textbf{-} \\ 
%         % car 9 & 1485.1 & - & 1366.0 & - & 1423.4 & - & 1459.6 & - & \textbf{1526.6} & \textbf{-} \\ 
%         % ferry 1 & 1454.3 & 0.3 & 1423.4 & - & 1441.5 & - & 1455.3 & - & \textbf{1492.6} & \textbf{-} \\ 
%         % ferry 10 & 1119.1 & 0.2 & 1021.3 & 0.2 & 1104.3 & 0.2 & 1104.3 & 0.2 & \textbf{1133.0} & \textbf{0.2} \\ 
%         % ferry 11 & 1038.3 & 1.2 & 847.9 & - & 978.7 & - & 1037.2 & 0.1 & \textbf{1067.0} & \textbf{-} \\ 
%         % ferry 12 & 1525.5 & - & 1324.5 & 6.4 & 1466.0 & - & 1555.3 & - & \textbf{1586.2} & \textbf{-} \\ 
%         % ferry 13 & 1421.3 & 0.5 & 1192.6 & 12.6 & \textbf{1320.2} & \textbf{-} & 1436.2 & 5.4 & 1471.3 & 1.8 \\ 
%         % ferry 14 & 2036.2 & - & 1850.0 & 0.3 & 2074.5 & - & 2098.9 & - & \textbf{2124.5} & \textbf{-} \\ 
%         % ferry 15 & 1551.1 & - & 1385.1 & - & 1535.1 & - & 1486.2 & 1.1 & \textbf{1573.4} & \textbf{-} \\ 
%         % ferry 16 & 2684.0 & - & 2406.4 & - & 2480.9 & - & 2734.0 & - & \textbf{2817.0} & \textbf{-} \\ 
%         % ferry 17 & 859.6 & 0.1 & 768.1 & 9.4 & 818.1 & - & 826.6 & - & \textbf{850.0} & \textbf{-} \\ 
%         % ferry 18 & 724.5 & 2.8 & 587.2 & 4.9 & 666.0 & 1.1 & 667.0 & 1.0 & \textbf{684.0} & \textbf{-} \\ 
%         % ferry 19 & 839.4 & 4.8 & 654.3 & - & \textbf{826.6} & \textbf{-} & 825.5 & - & 863.8 & 7.1 \\ 
%         % ferry 2 & 1012.8 & 3.3 & 951.1 & 10.6 & 990.4 & - & 1001.1 & - & \textbf{1024.5} & \textbf{-} \\ 
%         \hline
%     \end{tabular}
%     %\end{small}
% \end{table*}


% \subsubsection{Additional Experiments}
% We list the experimental details under validation dataset in Table~\ref{detail:1}, where the ABR algorithm includes Zwei, BOLA, RobustMPC, Pensieve and Rate-based. The validation set contains several different network scenarios. E.g., \emph{bus-1} represents network trace No.1 which collected from the bus.  

\subsection{CLS Scheduling}
\label{sec:cls}
% In this part, we evaluate Zwei in CLS scheduling task and compare it with several state-of-the-art scheduling algorithms.
% Results illustrate that Zwei is able to leverage historical CDN information for providing the live video streaming service with less number of blocked~(or stalling) users as well as lower CDN costs.


% \begin{figure}
% 	\centering
%   	\includegraphics[width=0.7\linewidth]{figs/cls}
%     \caption {CLS System overview.}
%     \label{fig:clsoverview} 
% \end{figure}

\begin{figure}
    \centering
    % \subfigure[Piece-wise Linear Model]{
    %     \includegraphics[width=0.23\linewidth]{figs/lts0}
    %     \label{fig:plm}
    % }\subfigure[Workload - Cost]{
    %     \includegraphics[width=0.23\linewidth]{figs/lts3}
    %     \label{fig:workloadcost}
    % }
    \subfigure[Zwei vs. Existing Methods]{
        \includegraphics[width=0.48\linewidth]{figs/lts1}
        \label{fig:clszwei}
    }\subfigure[Zwei Training Curve]{
        \includegraphics[width=0.48\linewidth]{figs/lts2}
        \label{fig:clstraining}
    }
    \vspace{-15pt}
    \caption{Results of Zwei under the CLS environment.}
    \vspace{-10pt}
    \label{fig:lts2}
\end{figure}

\subsubsection{CLS Overview}
% A typical CLS system is illustrated in Figure~\ref{fig:clsoverview}. 
The ClS system is composed of a source server and several CDNs. Upon received viewers' requests, the CLS platform will first aggregate all stream data to the source server, and then deliver the video stream to viewers through CDN providers according to a certain scheduling strategy.
% This figure shows that viewer A, B, and C are watching broadcaster a, b,and c through CDN A, CDN B, CDN B, respectively.
\vspace{-5pt}
\subsubsection{Implementation}
Our experiments are conducted on the real-world CLS dataset provided by the authors~\cite{zhang2019enhancing}, spanning 1 week (6 days for training and 1 day for test). At each time, we select 3 candidates from total 4 different CDN providers, and we fit a separate simulator for them. Followed by previous work~\cite{zhang2019enhancing}, we use a piecewise linear model to characterize this relationship between workload and block ratio. Note that the following features are extracted by the real CDN dataset. What's more, we set the CDN pricing model w.r.t various CDN providers in industry, such as Amazon E2 and Tencent CDN. See~\cite{zweigit} for details.
\vspace{-5pt}

\begin{small}
\begin{algorithm}
\caption{Rule for the CLS task.} 
\label{alg:Overallcls} 
\begin{algorithmic}[1]
\Require Trajectory $T_{u}, T_{v}$;
\State Compute average stalling ratio ${stall}_{u}, {stall}_{v}$, accumulative cost $c_{u}, c_{v}$ from the given trajectories $T_{u}, T_{v}$. \Comment Requirements: i) low stalling ratio ii) low costs.
\State Initialize Return $s=\{-1, -1\}$;
\If{$\left| {stall}_{u} - {stall}_{v} \right|< \epsilon$ or $\left| c_{u} - c_{v} \right|< \epsilon_{c}$}
\State Randomly set $s_{0}$ or $s_{1}$ as 1. 
\Comment Add noise to improve the robustness.
\ElsIf{$\left| {stall}_{u} - {stall}_{v} \right|<\epsilon_{c}$}
\State $s_i \gets 1, i={argmin}_{i\in \{u,v\}}{c}$;
\Else
\State $s_i \gets 1, i={argmin}_{i\in \{u,v\}}{stall}$;
\EndIf
\State return $s$;
%\EndProcedure
\end{algorithmic} 
\end{algorithm}
\end{small}
\vspace{-10pt}
\textbf{Baselines.}
Like other scenarios, we also compare Zwei with the following state-of-art scheduling baselines:
\begin{enumerate}[leftmargin=*]
    \item \textbf{\emph{Weighted round robin~(WRR)}~\cite{adhikari2012unreeling}.} The requests will be redirected to different CDN providers w.r.t a constant ratio. We adopt the algorithm with the \emph{best} parameters.

    \item \textbf{\emph{E2}~\cite{jiang2017pytheas}.}~Exploitation and Exploration~(E2) algorithm utilizes harmonic mean for estimating CDN providers' performance, and select with the highest upper confidence bound of reward. We use E2 algorithm provided by the authors~\cite{jiang2017pytheas}.
    
    \item \textbf{\emph{LTS}~\cite{zhang2019enhancing}.}~State-of-the-art CLS algorithm which uses deep reinforcement learning to train the NN towards lower stalling ratio. However, it ignores the trade-off between the cost and the performance. We evaluate LTS by Zhang et. al.~\cite{zhang2019enhancing}.
\end{enumerate}

\textbf{NN Representation.}
We implement Zwei in CLS as suggested by recent work~\cite{zhang2019enhancing}. More precisely speaking, for each CDN provider $i$, Zwei passes past 20 normalized workload and stalling ratio into Conv-2D layers with filter=64, size=4, and stride=1. Then several output layers are merged into a hidden layer that uses 64 units to apply the \emph{softmax} activation function. We model the action space as a heuristic way: each CDN provider has 3 choices, i.e., incrementally increases its configuration ratio by 1\%, 5\%, and 10\%. 

\textbf{Requirements for CLS tasks.}
Algorithm~\ref{alg:Overallcls} describes the $\texttt{Rule}$ of CLS. Note that the $\epsilon_{c}=10$ is also a small number that can add noise to improve Zwei's robustness.

\textbf{Zwei vs. State-of-the-art Scheduling Methods}
We start to study how well that Zwei achieves under the CLS scenario. As shown in Figure~\ref{fig:clszwei}, we find that Zwei stands for the best scheme among the candidates. Specifically, Zwei reduces the overall costs on 22\% compared with state-of-the-art learning-based method LTS, and decreases over 6.5\% in terms of the overall stalling ratio. The reason is that LTS takes the weight-sumed combination function as the reward, while the function can hardly give a clearer guidance for the optimized algorithm. Moreover, comparing the performance of Zwei with the optimal strategy generated by the reward function, we observe that both optimal policy and Zwei are in the Pareto front. Zwei consumes less pricing costs than the optimal policy since the requirement is to \emph{minimize the cost first}.

\textbf{Details.}
Besides, we also present the training process in Figure~\ref{fig:clstraining}. As shown, Zwei converges in less than 600 epochs, which needs about 3 hours. It's worth noting that Zwei also experienced two stages on the CLS task. The first stage ranges from 0 to 100 epochs, and we can see the goal of Zwei is to minimize the cost without considering the number of stalling ratio. The rest of the process we find that Zwei attempts to reduce the number of stalling ratio. Meanwhile, the cost curve converges to a steady state. 
% Such observation also proves that Zwei learns the strategies by following the given requirements.
%2540.34532224,5649.002271424225

% \subsection{RTC Tasks}
% \label{sec:rtc}
% To better understand how Zwei performs in the RTC task, we further develop a faithful packet-level network emulation testbed, train Zwei via various real-world network traces, and validate Zwei with scale. As expected, results also prove the superiority of Zwei against existing methods.
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.95\linewidth]{figs/rtc}
% %     \caption{RTC System Overview.}
% %     \label{fig:rtcoverview}
% % \end{figure}

% \noindent \textbf{RTC Overview}
% % We start with explaining the conventional end-to-end transmission process for real-time video streaming. As shown in Figure~\ref{fig:rtcoverview}, t
% The RTC system contains a sender and a receiver, and its transport protocol mainly consists of two channels: the streaming channel and the feedback message channel. At the beginning, the sender deploys a UDP socket channel to send the instant real-time video streaming packets $P = \{p_0,p_1,\cdots,p_k\}$ to the receiver through the streaming channel. The receiver then feeds network status observed back to the sender through the feedback channel. Based on this information, the sender will select bitrate for next time period.

% % \subsubsection{Network Simulator Setup}
% % \label{sec:simulator} 
% % In this part, we aim to introduce the principle of the RTC network simulator. To train Zwei in the RTC scenario, we first consider training the neural network~(NN) model in real-world network conditions, i.e., deploying the model on the edge server. The model will finally converge with the increased number of video session. However, it's hard to converge since online training should explore almost all network status. We then decide to train the model in simulated offline networks. Hence, we are facing a new challenge: \emph{how to design a fast-forward network simulator which can precisely compute the latency with given saturated trace and sending rate?} 

% % % Thus, we consider one-way delay, a metric that is widely used in congestion control algorithm. One-way delay consists of transmission delay, queuing delay and random noise. Predicting one-way delay requires detailed information for each router on the channel link between a sender and receiver. However, for each router on the session, there is always a special strategy with its own status and routing algorithms that we cannot collect. As a result, we can't estimate the accurate delay metrics in the offline environment with the parameters collected through our protocol.

% % We adopt delay gradient instead of one-way delay to train Zwei. Delay gradient is defined as the difference on delay measurement on both side.~\cite{carlucci2016analysis} It is also proposed to measure the latency in un-synchronized clock environment. Delay gradient $q(t_i)$ is computed as Eq.~\ref{eq: gradient}, which is actually used to describe the variety of the queuing delay. If the network is congested, its delay gradient will be greater than zero, vice versa. If the delay gradient equals to zero, we can only infer that network is not congested.
% %  \begin{align}
% %  \begin{aligned}
% %  q(t_i) = \frac{1}{N}\sum\limits_{i=1}^{N}\left[(t_i-t_{i-1})-(T_i-T_{i-1})\right]
% %  % =\frac{1}{N}{(t_1 - T_{N-1})}
% %     \label{eq: gradient} 
% %  \end{aligned}
% %  \end{align}
% % Where $T_i$ is the time at which the i-th packet has been sent, and $t_i$ is the time at which the i-th packet has been received, and N represents the packet count in a period. %However, in real-world network environment, delay gradient is often observed along with burst noise. %In our study, we filter the noise by a complementary filter.

% % Our simulator should emulate the process of the packets coming and leaving in different network conditions, and keep track of the timestamps, by which we are able to obtain the corresponding queuing delay gradient. Inspired by recent work~\cite{winstein2013stochastic}, we utilize saturated network trace to generate queuing delay data. As shown in Figure~\ref{fig:queue}, assuming the distribution of packets arrival and leave fits closely to the Poisson process~\cite{winstein2013stochastic}, we use sending bitrate and bandwidth in saturated network traces as the arriving rate $\lambda$ and leaving rate $\mu$, respectively.

% % In detail, we regard the channel link between the sender and the receiver as a single device. The device is comprised of three queues, namely \emph{input}, \emph{output} and \emph{limbo}. An algorithm is designed to release packets from each queue corresponding to the network trace dataset in different levels. Each element in the queue is the opportunity of packet-delivery, which means, the time~(in milliseconds) at which an MTU-sized packet will be delivered. For each period $(t_k,t_{k+1}]$, the offline-network simulator compares the timestamp of the front packet in \emph{input} with that in \emph{limbo}. If timestamp in \emph{input} queue is bigger than or equal to the one in \emph{limbo}, the simulator will push the front packet into the bottom of the \emph{output} queue, and then computes the delay gradient between the two packets. On the contrast, the delivery opportunities will be wasted if the timestamp in \emph{input} queue is smaller than that one in \emph{limbo} queue. The simulator only pops the front packet in \emph{limbo} queue. By this process, the simulator returns mean self-inflicted delay and total bytes that the sum of \emph{output} queue every interval $t_{k+1} - t_{k}$.

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.7\linewidth]{figs/limbo}
% %     \caption{The working principle of the network simulator.}
% %     \label{fig:queue} 
% % \end{figure}

% \noindent \textbf{NN Architecture Overview}
% We use past $k=10$ sequence, and for each sequence we take past sending rate, past receive rate, delay gradient, round-trip time~(RTT), loss ratio as the input. Besides, we output the NN as 11-dims vector $a$ to control the sending rate, which represents \{-0.4, -0.3, -0.2, -0.1, -0.05, 0.0, 0.05, 0.1, 0.2, 0.3, 0.4\}. Inspired by the additive-increase, multiplicative-decrease~(AIMD) algorithm, we take different logic to increase or decrease the sending rate. Zwei increases the sending rate $r_t$ as $r_t=r_t+r_{max} \times a_{t}$, and reduces the sending rate as $r_t=r_t \times (1-a_t)$. We set minimum sending rate $r_{min}=0.01$ and $r_{max}=4mbps$. '
% Like previous work~\cite{QARC2018}, we use the combination of 1D-CNN and Fully connected layers to extract the feature and then merge into a vector.

% \noindent \textbf{Experimental Setup}
% We develop a faithful network emulator which can simulate the network condition according to network saturate traces that collected from different network conditions. The network traces is composed of 3G, 4G/LTE and WiFi network as well as self-collected real-world network environments. We then train Zwei under the simulator for about 8 hours and validate it with the baseline methods over another traces.


% \textbf{RTC Baselines}
% We compare Zwei with several baselines.
% \label{sec:rtcbaseline}
% \begin{enumerate}[leftmargin=*]
%     \item \textbf{\emph{TCP}~\cite{mo1999analysis}}. The most popular congestion control algorithm in the Internet. The key insight is the additive-increase, multiplicative-decrease~(AIMD) algorithm, which means a linear increasing of the congestion window with an exponential reduction when congestion is detected. We adopt TCP-Reno with \emph{fast recovery}.% for this experiment.
%     \item \textbf{\emph{WebRTC}~\cite{carlucci2016analysis}}. The state-of-the-art RTC scheme on both academic and industry. More precisely speaking, WebRTC leverage delay-based and loss-based module to jointly control the rate adaption problem in the real-time scenario, where its parameters have been carefully tuned for almost one decade.
% \end{enumerate}

% % \begin{figure}
% % 	\centering
% %   	\includegraphics[width=0.48\linewidth]{figs/rtc0}
% %   	\includegraphics[width=0.48\linewidth]{figs/rtc1}
% %     \caption{RTC System Overview. We implement the system suggested by prior research~\cite{QARC2018,carlucci2016analysis}.}
% %     \label{fig:rtc}
% % \end{figure}

% % TCP,0.360592172299,0.536535959977,1.51068102901
% % WebRTC,0.238234762662,0.205969435567,0.977550851188
% % Zwei,0.26594276212988605,0.1636653622608551,0.3618892683769965

% % TCP,0.404259912862,0.273416227453,460.976099842
% % WebRTC,0.324406768074,0.138330459595,368.640693226
% % Zwei,0.36361010757437784,0.1453350397892771,318.3359234234234



% \noindent \textbf{Zwei vs. RTC Baselines}
% In this experiment, we compare Zwei with existing proposed heuristic methods~(\S\ref{sec:rtcbaseline}) on various network conditions such as 3G and Wifi. We collect average receiving bitrate, 95 percent RTT, and average loss ratio per second. Note that these metrics are widely used in RTC evaluation~\cite{QARC2018}. Results are reported in Figure~\ref{fig:rtc}, we demonstrate that Zwei improves 11.34\% on average receiving bitrate, reduces 20.49\% in terms of loss ratio, and decreases 62.95\% on 95-percent RTT compared with WebRTC under HSDPA dataset. Another results on the WiFi network conditions show that Zwei also outperforms WebRTC, with the improvements on sending rate of 12.08\% and decreasing in 95\% RTT of 13.59\%. The comparison result indicates that Zwei can effectively detect the congestion signal and dynamically adjust the sending rate to avoid high loss ratio and RTT.


% \begin{figure}
%     \centering
%     \subfigure[HSDPA]{
%             \includegraphics[width=0.48\linewidth]{figs/rtc0}
%     }\subfigure[WiFi]{  
%         \includegraphics[width=0.48\linewidth]{figs/rtc1}
%     }
%     %\vspace{-10pt}
%     \caption{The comparison of Zwei and WebRTC as well as TCP on both HSDPA and WiFi network datasets.}
%     \label{fig:rtc}
% \end{figure}


% \subsubsection{Zwei Case Study}
% To better understand the performance of the selected methods, we \textbf{randomly} pick four traces from the validation dataset and compare the sending rate curve of Zwei with TCP and WebRTC. As demonstrated in Figure~\ref{fig:rtc2} and Figure~\ref{fig:rtc3}, Zwei can accurately estimate the bottleneck of the session, as it always sends video streaming with high rate with avoiding congestion. 
% % Results of the rest of validation network traces are listed in \textbf{\emph{supplementary materials}}.


% \begin{figure*}
%     \centering
%     \subfigure[Available Bandwidth]{
%         \includegraphics[width=0.245\linewidth]{all/abw-norway-car-2}
%     }\subfigure[TCP]{
%             \includegraphics[width=0.245\linewidth]{all/tcp-norway-car-2}
%     }\subfigure[WebRTC]{
%             \includegraphics[width=0.245\linewidth]{all/webrtc-norway-car-2}
%     }\subfigure[Zwei]{
%             \includegraphics[width=0.245\linewidth]{all/zwei-norway-car-2}
%     }
    
%     % \subfigure[Available Bandwidth]{
%     %     \includegraphics[width=0.245\linewidth]{all/abw-norway-bus-14.png}
%     % }\subfigure[TCP]{
%     %     \includegraphics[width=0.245\linewidth]{all/tcp-norway-bus-14.png}
%     % }\subfigure[WebRTC]{
%     %     \includegraphics[width=0.245\linewidth]{all/webrtc-norway-bus-14.png}
%     % }\subfigure[Zwei]{
%     %     \includegraphics[width=0.245\linewidth]{all/zwei-norway-bus-14.png}
%     % }
%     %\vspace{-10pt}
%     \caption{The comparison of Zwei and existing methods on the HSDPA network trace.}

%     \label{fig:rtc2}

%     \subfigure[Available Bandwidth]{
%         \includegraphics[width=0.245\linewidth]{all/abw-12320-wifi5}
%     }\subfigure[TCP]{
%             \includegraphics[width=0.245\linewidth]{all/tcp-12320-wifi5}
%     }\subfigure[WebRTC]{
%             \includegraphics[width=0.245\linewidth]{all/webrtc-12320-wifi5}
%     }\subfigure[Zwei]{
%             \includegraphics[width=0.245\linewidth]{all/zwei-12320-wifi5}
%     }
%     % \subfigure[Available Bandwidth]{
%     %     \includegraphics[width=0.245\linewidth]{all/abw-trace-3.png}
%     % }\subfigure[TCP]{
%     %     \includegraphics[width=0.245\linewidth]{all/tcp-trace-3.png}
%     % }\subfigure[WebRTC]{
%     %     \includegraphics[width=0.245\linewidth]{all/webrtc-trace-3.png}
%     % }\subfigure[Zwei]{
%     %     \includegraphics[width=0.245\linewidth]{all/zwei-trace-3.png}
%     % }
%     %\vspace{-10pt}
%     \caption{We also compare Zwei with existing methods on the trace collected from the real-world WiFi scenario.}
        
%     \label{fig:rtc3}
% \end{figure*}


==> Zwei 4/ieee.tex <==
%\documentclass[10pt, letterpaper]{IEEEtran}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{comment}
\usepackage{color}
\usepackage{amsmath}
%\usepackage{subcaption}
\usepackage{booktabs} 
% For formal tables
\usepackage{multirow}
\usepackage{algorithm}
\usepackage{array}
\usepackage{enumitem}
\usepackage[noend]{algpseudocode}
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\PassOptionsToPackage{hyphens}{url}
%\usepackage{hyperref}
\usepackage[export]{adjustbox}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{colortbl}
\definecolor{mygray}{gray}{.9}
\usepackage{euscript}
\usepackage{amssymb}
\usepackage{algorithm,algpseudocode}
\usepackage{framed}
%\usetikzlibrary{automata, positioning, arrows, shapes}
\renewcommand{\arraystretch}{1.25}
\newcommand{\dtoprule}{\specialrule{1pt}{0pt}{0.4pt}%
\specialrule{0.3pt}{0pt}{\belowrulesep}%
}
\newcommand{\dbottomrule}{\specialrule{0.3pt}{0pt}{0.4pt}%
\specialrule{1pt}{0pt}{\belowrulesep}%
}

% colorful citation
 \usepackage{color}
 \usepackage{hyperref}
 \definecolor{darkred}{rgb}{0.6,0,0}
 \definecolor{darkgreen}{rgb}{0,0.5,0}
 \definecolor{darkblue}{rgb}{0,0.0,0.3}
 \hypersetup{colorlinks=true,
 		 %urlcolor=darkblue,
         linkcolor=darkred,
         citecolor=darkgreen
         }

\newcommand{\up}[1]{#1{}{\color{darkgreen}$\uparrow$}}
\newcommand{\down}[1]{#1{}{\color{darkred}$\downarrow$}}
         
% Compact itemize and enumerate.
\def\compactify{\itemsep=0pt \topsep=0pt \partopsep=0pt \parsep=0pt}
\let\latexusecounter=\usecounter
\newenvironment{CompactItemize}
  {\def\usecounter{\compactify\latexusecounter}
   \begin{itemize}\setlength{\leftmargin}{1.0em}}
  {\end{itemize}\let\usecounter=\latexusecounter}
\newenvironment{CompactEnumerate}
  {\def\usecounter{\setlength{\leftmargin}{1.75em}\compactify\latexusecounter}
   \begin{enumerate}}
  {\end{enumerate}\let\usecounter=\latexusecounter}        
%
% If IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it like:
% \documentclass[journal]{../sty/IEEEtran}





% Some very useful LaTeX packages include:
% (uncomment the ones you want to load)


% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.






% *** CITATION PACKAGES ***
%
%\usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.






% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex





% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath





% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.




% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig




% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix




%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
% endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% Axel Sommerfeldt. This package may be useful when used in conjunction with 
% IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% submissions have lists of figures/tables at the end of the paper and that
% figures/tables without any captions are placed on a page by themselves at
% the end of the document. If needed, the draftcls IEEEtran class option or
% \CLASSINPUTbaselinestretch interface can be used to increase the line
% spacing as well. Be sure and use the nomarkers option of endfloat to
% prevent endfloat from "marking" where the figures would have been placed
% in the text. The two hack lines of code above are a slight modification of
% that suggested by in the endfloat docs (section 8.4.1) to ensure that
% the full captions always appear in the list of figures/tables - even if
% the user used the short optional argument of \caption[]{}.
% IEEE papers do not typically make use of \caption[]'s optional argument,
% so this should not be an issue. A similar trick can be used to disable
% captions of packages such as subfig.sty that lack options to turn off
% the subcaptions:
% For subfig.sty:
% \let\MYorigsubfloat\subfloat
% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% However, the above trick will not work if both optional arguments of
% the \subfloat command are used. Furthermore, there needs to be a
% description of each subfigure *somewhere* and endfloat does not add
% subfigure captions to its list of figures. Thus, the best approach is to
% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% and instead reference/explain all the subfigures within the main caption.
% The latest version of endfloat.sty and its documentation can obtained at:
% http://www.ctan.org/pkg/endfloat
%
% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% later in the document, say, to conditionally put the References on a 
% page by themselves.




% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.




% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


\usepackage{dutchcal}
\begin{document}
%
% paper title
% Titles are generally capitalized except for words such as a, an, and, as,
% at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% not capitalized unless they are the first or last word of the title.
% Linebreaks \\ can be used within to get better formatting as desired.
% Do not put math or special symbols in the title.
\title{Learning Video Transmission Algorithms via Requirements}
%
% learning to generate strategies for various video transmission tasks via self-play reinforcement learning
% author names and IEEE memberships
% note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% a structure at a ~ so this keeps an author's name from being broken across
% two lines.
% use \thanks{} to gain access to the first footnote area
% a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% was not built to handle multiple paragraphs
%
\author{Tianchi Huang, Rui-Xiao Zhang, Lifeng Sun
% <-this % stops a space
\thanks{Corresponding Author: Lifeng Sun, mailto: sunlf@tsinghua.edu.cn.}%
\thanks{Media Lab, Tsinghua University.}
\thanks{Manuscript received July 21, 2019; revised Oct. 26, 2019.}
}

% note the % following the last \IEEEmembership and also \thanks - 
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
% 
% \author{....lastname \thanks{...} \thanks{...} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.



% The paper headers
%\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
%{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% The only time the second header will appear is for the odd numbered pages
% after the title page when using the twoside option.
% 
% *** Note that you probably will NOT want to include the author's ***
% *** name in the headers of peer review papers.                   ***
% You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% you desire.




% If you want to put a publisher's ID mark on the page you can do it like
% this:
%\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.



% use for special paper notices
%\IEEEspecialpapernotice{(Invited Paper)}




% make the title area
\maketitle

% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\input{abs}
% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Video transmission Strategy, Reinforcement Learning, Adaptive Bitrate Streaming.
\end{IEEEkeywords}






% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

\input{intro}
\input{preliminaries}
\input{method}
\input{eval}
\input{related}
\input{conclusion}

% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
\newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
\bibliography{ref}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
% \begin{thebibliography}{1}
%\input{sample-sigconf.bbl}
% \begin{thebibliography}{1}

% \bibitem{IEEEhowto:kopka}
% H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%   0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

% \end{thebibliography}

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
% \newpage
% \begin{IEEEbiography}{Tianchi Huang}
% received his M.E degree in the Department of Computer Science and Technology in Guizhou University in 2018. Currently he is a Ph.D student in the Department of Computer Science and Technology at Tsinghua University, advised by Prof. Lifeng Sun. 

% His research work focuses on the multimedia network streaming, including transmitting streams, overlay path construction and edge-assisted content delivery. He received Best Student Paper Awards presented by ACM Multimedia System 2019 Workshop.
% \end{IEEEbiography}

% \begin{IEEEbiography}{Rui-Xiao Zhang}
% received his B.E degree in Electronic Engineering Department in Tsinghua University in 2017. Currently, he is pursuing his Ph.D candidate in Department of Computer Science and Technology, Tsinghua University, China. 

% His research interests lie in the area of content delivery networks, the optimization of multimedia streaming and cloud computing. He received Best Student Paper Awards presented by ACM Multimedia System 2019 Workshop.
% \end{IEEEbiography}

% \begin{IEEEbiography}{Lifeng Sun}
% received the B.S and Ph.D degrees in system engineering from National University of Defense Technology, Changsha, Hunan, China, in 1995 and 2000, respectively. He joined Tsinghua University since 2001.
% He is currently a Professor with the Computer Science and Technology Department of Tsinghua University, Beijing.

% Dr.Sun's research interests include the area of networked multimedia, video streaming, 3D/multiview video coding, multimedia cloud computing, and social media.
% \end{IEEEbiography}

% if you will not have a photo at all:

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks
\end{document}




==> Zwei 4/intro.tex <==
\section{Introduction}
Thanks to the dynamic growth of video encoding technologies and basic Internet services~\cite{cisco}, currently we are living with the great help of video transmission services. 
% Users often watch interesting videos and live streaming from different video content providers~(e.g. YouTube and Kuaishou), or chat with each other via real-time video communication rather than a conventional phone call. In such scenarios, 
In particular, the videos are required to transmit with fulfilling users' requirements, where the requirement is often known as quality of experience~(QoE) or quality of service~(QoS).
% high bitrate and less rebuffering time or stalling ratio. However, due to the fluctuation and unpredictability of network conditions, blindly achieving high bitrate may heavily increase the probabilities of the rebuffering event. 
% Hence, several rate adaptation methods are proposed to take these factors into consideration. 
% Further, from the video content provider's perspective, they aim to provide video streaming services with less stalling ratio but lower costs, where it's also necessary to trade off the stalling ratio against the cost. 
% Thus, the services are required to employ scheduling algorithms for balancing the two.
% Thus, such aforementioned observations are being left on the horns of a classic dilemma: in the video transmission tasks, both quality of experience~(QoE) and quality of service~(QoS) are evaluated with contradicted metrics~(\S\ref{sec:background}). Hence, how to generally bridge the gap between these factors?
Unfortunately, as much as the fundamental issue has already been published about \emph{two decades}~\cite{mo1999analysis}, current approaches, either heuristics or learning-based methods, fall short of achieving this goal. 
On the one hand, heuristics often use existing domain knowledge~\cite{mo1999analysis} as the working principle. However, such approaches sometimes require careful tuning and will backfire under the circumstance that violated with presumptions, finally resulting in the failure of achieving acceptable performance under all considered scenarios. On the other hand, learning-based methods~\cite{mao2017neural,zhang2019enhancing} leverage deep reinforcement learning~(DRL) to train a neural network~(NN) by interacting with the environments without any presumptions, aiming to obtain higher reward. In recent work, the reward function is often defined as a linear-based equation with the combination of manipulation variables. 
% Unsurprisingly, the learned policy outperforms heuristics, with the improvements on the overall performance of more than 18\%~\cite{akhtar2018oboe}. 
While in this study, we empirically discover that i) an inaccurate reward function may mislead the learning-based algorithm to generalize bad strategies, since ii) the actual requirement can hardly be presented by the linear-based reward function with fixed weights. Moreover, iii) considering the diversity of real-world network environments, it's difficult to present an accurate reward function that can perfectly fit \emph{any} network conditions~(\S\ref{sec:challenges}). 
As a result, despite its abilities to gain higher numerical reward score, learning-based schemes may generalize a strategy that hardly meet the actual requirements.

Taking a look from another perspective, we observe that the aforementioned problem can be naturally described as a deterministic goal or requirement~\cite{huang2018tiyuntsong}. 
For instance, in the most cases, the goal of the adaptive bitrate~(ABR) streaming algorithm is to achieve lower rebuffering time first, and next, reaching higher bitrate~\cite{Huang2019Hindsight, mao2019real}. 
% It is pretty straightforward that it can be easily understood and refined by others.
% To this end, we attempt to train the NN based on the assigned requirement without reward engineering.
% Unfortunately, off-the-shelf learning-based algorithms are unable to optimize the policy like this since it lacks the abilities to provide any gradients information to guide the algorithm towards a better performance directly.
% Hence, we ask if self-play learning~\cite{alphazero2017} can help taming the complexity of video transmission services with the actual requirement and especially, without reward engineering. 
Inspired by this opportunity, we envision a self-play reinforcement learning-based framework, known as Zwei, which can be viewed as a solution for tackling the video transmission dilemma~(\S\ref{sec:design}).
The key idea of Zwei is to sample trajectories repeatedly by itself, and distinguish the sequence that is closer to the assigned demand, so as to learn the strategy for satisfying the demand iteratively. 
Specifically, we apply Monte-Carlo~(MC) search to estimate moving decisions from the starting point. In the MC search process, several trajectories are sampled from the starting state according to the current policy. Then the expected long-term win rate is estimated by averaging the competition results from each trajectory pairs, where the result represents which one is closer to the actual demand between the two trajectories.
Having estimated the win rate, Zwei adopts the proximate policy optimization~(PPO)~\cite{schulman2017proximal} to optimize the NN via increasing the probabilities of the winning sample and reducing the possibilities of the failure sample.

In the rest of the paper~(\S\ref{sec:eval}), we attempt to evaluate the potential of Zwei using trace-driven analyses of various representative video transmission scenarios. To achieve this, we build several faithful video transmission simulators which can accurately replicate the environment via real-world network dataset. Specifically, we validate Zwei on two different tasks~(\S\ref{sec:background}), including client-to-server, and server-to-client service. Note that each of them has individual requirements and challenges. As expected, evaluation results demonstrate the superiority of Zwei against existing state-of-the-art approaches on all tasks. In detail, we show that \textbf{(i)} Zwei outperforms existing ABR algorithms on both HD videos and 4K videos, with the improvements on Elo score~\cite{coulom2008whole} of 32.24\% - 36.38\%. 
\textbf{(ii)} In the crowd-sourced live streaming~(CLS) scheduling task, Zwei reduces the overall costs on 22\% and decreases over 6.5\% on the overall stalling ratio in comparison of state-of-the-art learning-based scheduling method LTS~\cite{zhang2019enhancing}. 
% \textbf{(ii)} Zwei generalizes well in the real-time communication~(RTC) scenario. Comparing the performance of Zwei and state-of-the-art heuristics WebRTC~\cite{carlucci2016analysis}, we observe that Zwei effectively improves 11.34\% on average receive rate, but reduces 20.49\% on loss ratio and 62.95\% on 95-percent round-trip-time~(RTT). 
% In particular, we find that Zwei perfectly follows the guidance of the given requirement since it demonstrates two distinct stages during the training process.

\noindent \textbf{Contributions: }This paper makes four key contributions.
\begin{itemize}[leftmargin=*]
    \item We point out the shortcoming of learning-based schemes in video transmission tasks and present the idea that update networks without reward engineering~(\S\ref{sec:challenges}). 
    \item Zwei is a novel framework that aims to employ the self-play reinforcement learning method to make the idea practical~(\S\ref{sec:design}).
    \item We implement Zwei into two representative video transmission scenarios, i.e. rate adaptation and crowd-sourced scheduling. Results indicates that Zwei outperforms existing schemes on all considered scenarios~(\S\ref{sec:eval}).
\end{itemize}

==> Zwei 4/method.tex <==
\section{Zwei Design}
\label{sec:design}
In this section, we briefly introduce the details of Zwei, including its key principle, training algorithms and implementation details. 

% \begin{align}
%     \label{eq:basic}
%     E(w^*)
% \end{align}

\begin{figure}
    \centering
    % \begin{minipage}{0.48\linewidth}
    %     \includegraphics[width=1.0\linewidth]{figs/0}
    % \end{minipage}
  	\includegraphics[width=0.8\linewidth]{figs/zweioverview}
  	\vspace{-10pt}
    \caption{Zwei System Overview. The framework is mainly composed of \emph{four} phases: Monte Carlo sampling, battle competition, win rate estimation, and policy optimization.}
    \label{fig:zweioverview}
\end{figure}

\subsection{Basic Idea}
\label{sec:selfplay}
% AlphaZero~\cite{silver2017mastering} is the most famous self-play algorithm who trains the NN solely based on an agent competes against the others. 
% To tackle the traditional RL methods' problem, we thereby consider following AlphaZero to train the algorithm via self-play RL. 
% The main idea of our proposed framework is to leverage these search operators repeatedly in a policy iteration procedure. 
% However, static games with incomplete information are much dissimilar and more complicated than dynamic games with complete information such as Go or Chess. 
% % Besides, recent self-play reinforcement learning methods use a Monte Carlo tree search~(MCTS) to provide a look-ahead search, where it often requires heavy computational costs. 
% Thus, we propose a novel self-play reinforcement learning framework, namely Zwei, aiming to tackle a critical challenge:~\emph{considering the specific features for video transmission task, how to design a proper general self-play reinforcement learning algorithm?}
As mentioned before, we attempt to generalize the strategy based on actual requirements instead of linear-based reward functions. Considering the basic requirement seldom directly provides gradients for optimization, we, therefore, employ the self-play method~\cite{silver2016mastering} that enables the NN to explore better policies and suitable rewards via self-learning.
Zwei treats the learning task as a competition between distinct trajectories sampled by itself, where the competition outcome is determined by a set of rules, symbolizing which one is closer to the given requirement. Subsequently, we are able to update the NN towards achieving a better outcome. 

\subsection{Training Methodology}
Figure~\ref{fig:zweioverview} presents the main phases in our framework. The pipeline can be summarized as follows: 

\textbf{Phase1: Monte Carlo Sampling.}~First, we adopt MC sampling method to sample $N$ different trajectories $T_{n}=\{s_{0}^n, a_{0}^n, s_{1}^n, a_{1}^n,$ $\dots, a_{t}^n\}, n \in N$ w.r.t the given policy $\pi(s)$ under the \emph{same environments}~($a_{t}\sim\pi(s_{t})$) and start point~(the gray point in Figure~\ref{fig:zweioverview}). Next, we record and analysis the underlying metric for the entire session. Finally, we store all the sample $T_{n}$ into $D$. Note that we can select Monte Carlo Tree Search~(MCTS)~\cite{silver2016mastering}, which is widely used in advanced research, to implement the process.

\textbf{Phase2: Battle Competition.}~To better estimate how the current policy performs, Zwei requires a module to label all trajectories from $D$: given two \emph{different} trajectories, $T_{i}$ and $T_{j}$ which are all collected from the \emph{same environment settings}~($T_{i}, T{j} \in D$)), we attempt to identify which trajectory is positive for NN updating, and which trajectory is generated by the worse policy. Thus, we implement a rule called $\texttt{Rule}$ which can determine the \emph{better} trajectory between the given two candidates, in which \emph{better} means which trajectory is closer to the requirement. At the end of the session, the terminal position $s_t$ is scored w.r.t the rules of the requirement for computing the game outcome $o$: $-1$ for a loss, $0$ for
a draw, and $+1$ for a win. The equation is listed in Eq.~\ref{eq:disc}. 
\begin{align}
    \label{eq:disc}
    o_{i}^{j} = \texttt{Rule}(T_{i}, T_{j}). \\
    s.t.\quad
    o_{i}^{j} = \{-1, 0, 1\}, T_{i}, T_{j} \in D, T_{i} \neq T_{j}.
\end{align}

\textbf{Phase3: Win Rate Estimation.}~Next, having computed the competition outcome $o_{i}$ for any two trajectories, we then attempt to estimate the average win rate $r_{i}$ for each trajectory $T_{i}$ in $D$, i.e., $r_{i} = \mathbb{E}[\texttt{Rule}(T_{i},)] = \lim_{N\to\infty}\frac{1}{N}\sum_{u}^{N} o_i^{u}$. Notice that the accuracy of the win rate estimation heavily depends on the number $N$ of trajectories. Since it's impractical to sample infinite number of samples in the real world, we further list the performance comparison of different sample numbers in \S\ref{sec:abr}.

% \begin{align}
%     \label{eq:Phase3}
%     r_{i} = \mathbb{E}[\texttt{Rule}(T_{i},)] = \lim_{N\to\infty}\frac{1}{N}\sum_{u}^{N} o_i^{u}.
% \end{align}

\textbf{Phase4: Policy Optimization.}~
In this part, given a batch of collected samples and their win rate, our key idea is to update the policy via \emph{elevating} the probabilities of the winning sample from the collected trajectories and \emph{diminishing} the possibilities of the failure sample from the worse trajectories. In other words, the improved policy $\pi$ at state $s_t$ is required to pick the action $a_t$ which produced the best estimated win rate $r_t$.
% , i.e., $a_t=argmax_{a}E[r_t(s_t, a)]$. 
% Hence, we can employ any policy gradient method~(e.g., A3C~\cite{mnih2016asynchronous}, TRPO~\cite{schulman2015trust}, ACKTR~\cite{wu2017scalable}) to optimize the NN's policy. 
We employ Proxy Policy Optimization (PPO)~\cite{schulman2017proximal}, a state-of-the-art actor-critic method, as to optimize the NN's policy. PPO uses clip method to restrict the step size of the policy iteration and update the NN by minimizing the following \emph{clipped surrogate objective}. We list the Zwei's loss function $\mathcal{L}^{\text{Zwei}}(\theta)$ in Eq.~(\ref{eq:adzwei}).
The function consists of a policy loss and a outcome loss. The policy are computed as Eq.~\ref{eq:policy}, 
where $p_t(\theta)$ denote the probability ratio between the policy $\pi_{\theta}$ and the old policy $\pi_{\theta_{\text{old}}}$, i.e.,  $\frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{\text{old}}}(a_t|s_t)}$; $ \epsilon$ is the hyper-parameters which controls the clip range. We set $\epsilon=0.2$ which consistent with the original paper~\cite{schulman2017proximal}. $\hat{A}_t$ is the advantage function~(Eq.~\ref{eq:advantage}),
$V_{\theta_{p}}(s)$ is provided by another value NN. 
Meanwhile, the value loss aims to minimize the mean square error between $r_t$ and $V_{\theta_{p}}(s)$~(Eq.~\ref{eq:value}). 
Moreover, we also add entropy $H(s_t; \theta)$ to encourage exploration. For more details, please refer to our repository~\cite{zweigit}. 
\begin{small}
\begin{align}
    \mathcal{L}^{\emph{Policy}}
    & = \hat{\mathbb{E}_{t}}\Big[ \min\Big( p_t(\theta)\hat{A}_t, \text{clip}\big(p_t(\theta), 1 - \epsilon, 1 + \epsilon\big)\hat{A}_t \Big) \Big]. 
    \label{eq:policy}
\end{align}
\begin{equation}
    \hat{A}_t = r_t - V_{\theta_{p}}(s_t)
    \label{eq:advantage}
\end{equation}

\begin{equation}
    \mathcal{L}^{\emph{Value}} = \frac{1}{2} \hat{\mathbb{E}_{t}}\left[ V_{\theta_{p}}(s_t) - r_t \right]^{2}.
    \label{eq:value}
\end{equation}

\begin{equation}
    \nabla \mathcal{L}^{Zwei} = \nabla_\theta \mathcal{L}^{\emph{Policy}} + \nabla_{\theta_{p}} \mathcal{L}^{\emph{Value}} + \nabla_\theta \beta H(s_t; \theta).
    \label{eq:adzwei}
\end{equation}
\end{small}
% \subsection{Training Methodology Overview}~Training procedure of Zwei is summarized in Algorithm~\ref{alg:Overall}. 
% % As shown, Zwei's workflow mainly consists of two parts, i.e., exploration and exploitation: 

% % \begin{enumerate}
% %     \item \emph{Exploration.} First, we sample $n$ trajectories roll-outed by the current policy in the same environment. Then we leverage $\texttt{Rule}$ to determine the better strategy via the pairwise comparison. Next, we estimate the win rate w.r.t the given samples.
% %     \item \emph{Exploitation.} We update the gradient by using the loss function $\mathcal{L}^{Zwei}$~(Eq.~\ref{eq:adzwei}).
% % \end{enumerate}
% \begin{small}
% \begin{algorithm}
% \caption{Zwei's Overall Training Procedure} 
% \label{alg:Overall} 
% \begin{algorithmic}[1]
% \Require Environment $\texttt{Env}$; Requirement $\texttt{Rule}$.
% \State Initialize parameters $\theta$ with random weights;
% \Repeat
% \State $\textit{D}=\{\}$; 
% \State $\texttt{Env} \gets $Sample environment settings;
% \For{$i \in \{1, 2, \dots, \textit{N}\}$}
% \Comment{MC search};
% \State Get state $s_t$ from $\texttt{Env}$.
% \State $\textit{T}_{i}=\{\}$;
% \While {not \textit{Terminal}}
% \State $a_t\sim\pi_\theta(s_t)$.
% \State $T_{i} \gets T_{i} \bigcup \{s_t, a_t\}$.
% \State Receive new state $s_{t+1}$
% \EndWhile
% \State $\textit{D} \gets \textit{D} \bigcup T_{i}$
% \EndFor

% \For{$pairs(T_u, T_v) \in \textit{D}$}
% \Comment{Battle competition};
% \State Determine win or loss: $o_{u}^{v} = \texttt{Rule}(T_{u}, T_{v})$;
% \EndFor

% \For{$T_u \in \textit{D}$}
% \Comment{Win rate estimation};
% \State Estimate win rate: $r_u=\frac{\sum_{i}^{N} o_{u}^{i}}{N}$.
% \For{$s_t, a_t \in T_u$}
% \Comment{Policy Optimization};
% \State Update NN with $\mathcal{L}^{Zwei}$~(Eq.~\ref{eq:adzwei});
% \EndFor
% \EndFor
% \Until{Converged}
% %\EndProcedure
% \end{algorithmic} 
% \end{algorithm}
% \end{small}
% \subsection{Parallel Training}
% \label{sec:parallel}
% During the training process, we observe that the training progress is inefficient while using a single process. Inspired by the multi-agent training method~\cite{mnih2016asynchronous}, we modify Zwei's training in the single agent as training in multi-agents. Multi-agents training consists of two parts, a central agent and a group of forwarding propagation agents. The forward propagation agents only decide with both policy and critic via state inputs and neural network model received by the central agent for each step; then it sends the $n$-dim vector containing $\{s, a, r\}$ to the central agent. The central agent uses the actor-critic algorithm to compute gradient and then updates its neural network model. Finally, the central agent pushes the updated network parameters to each forward propagation agent. Note that this can happen asynchronously among all agents, for instance, there is no locking between agents. By default, Zwei employs 12 forward propagation agents and one central agent.



==> Zwei 4/preliminaries.tex <==
% \begin{figure}
% 	\centering
%       \includegraphics[width=0.9\linewidth]{figs/main2}
%     \caption{A brief introduction of today's video transmission service. As shown, the service is mainly composed of client-to-server, server-to-client and client-to-client services~(\S\ref{sec:background}).}
%     \label{fig:system}
% \end{figure}

\section{Background and Challenges}
\label{sec:back}
% In this section, we first normally introduce the background of adaptive video streaming scenarios, including client-to-server, server-to-client, and client-to-client service, and then we briefly elaborate the key challenges of each service. 

\subsection{Video Transmission Services}
\label{sec:background}
% To better understand the limitations that conventional video streaming service suffering from, we plot the general service work-flow on Figure~\ref{fig:system}. 
% We summarize the task name, task features, requirement and constrains for each video transmission scenario in Table~\ref{tbl:req}. 
In this work, the video transmission service mainly consists of:

\textbf{\emph{Client-to-Server Service.}}~In this scenario, users often adopts a video player to watch the video on demand. First, video contents are pre-encoded and pre-chunked as several bitrate ladders on the server. Then the video player, placed on the client side, dynamically picks the proper bitrate for the next chunk to varying network conditions. Specifically, the bitrate decisions should achieve high bitrate and low rebuffering on the entire session~\cite{bentaleb2018survey,Huang2019Hindsight}. We call it \emph{adaptive bitrate streaming}~(ABR).
    
\textbf{\emph{Server-to-Client Service.}}~Considering that if we were the content provider and currently we had multiple content delivery networks~(CDNs) with different costs and performance, how to schedule the users' requests to the proper CDN, aiming to provide live streaming services withing less stalling ratio and lower cost? In common, we call that \emph{crowd-sourced live streaming(CLS)}~\cite{zhang2019enhancing}.
    
% \textbf{\emph{Client-to-Client Service.}}~Besides, in our daily life, we usually chat with other users instantly via a video call namely \emph{Real-Time video Communication~(RTC)}. The RTC system consists of a sender and a receiver. The sender deploys a UDP socket channel and sends the encoded video packets to the receiver. The receiver then feeds the messages back to the sender through feedback channel. During the session, the sender adjusts the sending bitrate for next time period, aiming to achieve high bitrate and low round-trip time~(RTT) as well as less loss ratio~\cite{QARC2018}.


% In general, we list the requirement and details for each video transmission task in Table~\ref{tbl:req}. Notice that we label the underlying metric orderly since each metric has attentive priority~(E.g, the priority of low rebuffering time is higher than that of high bitrate in the ABR scenario). 
Details of each video transmission scenario are demonstrated in \S\ref{sec:eval}. We can see that the video transmission task is often required to obtain better performance under various mutual metrics.
% which makes the key principle of designing a traditional networking algorithm: best-effort delivery~\cite{lefelhocz1996congestion}. While learning-based approaches pursue best-performance delivery, aiming to maximize the overall performance over all considered networks. To this end, what's the Achilles' heel of the best-performance approach?



% \begin{table}[]
%     \centering
%     \caption{Requirements for each video transmission tasks.}
%     \label{tbl:req}
%     \begin{tabular}{c|c|c}
%         \hline
%         Transmission Type & Is ABR? & Requirement \\ \hline
%         \emph{\textbf{Client-to-Server}}  & \checkmark              & \down{Rebuffering Time$^1$}, \up{Bitrate$2$} \\
%         \emph{\textbf{Server-to-Client}}  & $\times$               & \down{Stalling Ratio$^1$}, \down{Cost$^2$} \\
%         \emph{\textbf{Client-to-Client}}  & \checkmark              & \down{RTT$^1$}, \down{Loss$^1$}, \up{Bitrate$^2$} \\ \hline
%     \end{tabular}
% \end{table}


\subsection{Challenges}
\label{sec:challenges}
% In this work, we aim to fuse the best-effort approach~(i.e., heuristics) and best-performance approach~(i.e., learning-based approach). 
\textbf{Motivation.}~Recent video transmission algorithms mainly consist of two types, i.e., heuristics and learning-based scheme. Heuristic methods utilize an existing fixed model or domain knowledge to construct the algorithm, while they inevitably fail to achieve optimal performance in all considered network conditions due to the inefficient parameter tuning~(\S\ref{related:heu},\cite{mao2017neural}). Learning-based schemes train a NN model towards the higher reward score from scratch, where the reward function is often defined as a linear combination of several weighted metrics~\cite{zhang2019enhancing, mao2017neural}. Nevertheless, considering the characteristics of the video transmission tasks above, \emph{we argue that the policy generated by the linear-based reward fails to always perform on the right track}. We, therefore, set up two experiments in the ABR scenario~(\ref{sec:abr}) to prove this conjecture. 
%The reason why we use this scenario to describe the challenges is that the ABR task is the easiest to understand and closest to the user in the video transmission scenario~\cite{cisco}.

\begin{figure}
  \centering
    \includegraphics[width=0.48\linewidth]{figs/norway_tram_24}
    \includegraphics[width=0.48\linewidth]{figs/norway_metro_8}
%\includegraphics[width=0.24\linewidth]{figs/log_sim_rl_norway_train_2}
%\includegraphics[width=0.31\linewidth]{figs/log_sim_rl_norway_train_19}
  	\vspace{-5pt}
    \caption{We show average bitrate and rebuffering time for each ABR method. ABRs are performed over the HSDPA network traces.}
  %\vspace{-20pt}
\label{fig:vmaf}
\end{figure}

%\noindent\rule[0.25\baselineskip]{\linewidth}{1pt}
%\begin{framed}
\noindent $\textbf{Observation 1.}$ \emph{The best learning-based ABR algorithm Pensieve~\cite{mao2017neural} is not always the best scheme on every network traces.}
%\end{framed}
%\noindent\rule[0.25\baselineskip]{\linewidth}{1pt}

Recently, given a deterministic QoE metric with linearly combining of several underlying metrics, several attempts have been made to propose the ABR algorithm via model-based~\cite{yin2015control} or model-free reinforcement learning~(RL) method~\cite{mao2017neural}. 
% E.g., RobustMPC~\cite{yin2015control} is a model-based RL approach which utilizes a solver~(e.g.~\texttt{CPLEX} or \texttt{Gurobi}) and a faithful offline ABR simulator to maximize QoE objectives by planning; Pensieve~\cite{mao2017neural} is a model-free RL approach which learns the system dynamic via interacting with the ABR environment.
However, such method heavily relies on the accuracy of the given QoE metric. Especially, \emph{how to set a proper QoE parameter for each network condition} is indeed a critical challenges for training a good ABR algorithm. In order to verify whether QoE parameters have influenced the performance of ABR algorithms, we set up an experiment to report average bitrate and rebuffering time of several state-of-the-art ABR baselines~(\S\ref{sec:abrbaseline}) and Zwei. Despite the outstanding performances that Pensieve achieves, the best learning-based ABR algorithm does not always stand for the best scheme. On the contrary, Zwei always outperforms existing approaches.

\begin{figure}
	\centering
  	\includegraphics[width=0.48\linewidth]{figs/opt0}
  	\includegraphics[width=0.48\linewidth]{figs/opt1}
  	\vspace{-5pt}
    \caption{The comparison of linear-based optimal and requirement-based optimal strategy. Results are evaluated on \emph{fixed~(0.5mbps)} and the real-world network trace~\cite{riiser2013commute}. We can see the difference between the actual requirement and the optimal trajectory generated by the linear-based reward.}
    \label{fig:case}
    \vspace{-15pt}
\end{figure}

%\noindent\rule[0.25\baselineskip]{\linewidth}{1pt}
%\begin{framed}
\noindent $\textbf{Observation 2.}$ \emph{Recent linear-based weighted reward function can hardly map the actual requirement for all the network traces.}
%\end{framed}
%\noindent\rule[0.25\baselineskip]{\linewidth}{1pt}

To better understand the effectiveness of weighted-sum-based reward functions, we compare the optimal strategy of linear-based with requirement-based under two representative network traces, in which linear-based optimal is the policy which obtains maximum reward, and the requirement-based optimal stands for the closest strategy in terms of the given requirement. Unsurprisingly, from Figure~\ref{fig:case} we observe that linear-based optimal policy performs differently compared with the requirement-based optimal strategy. The reason is that the given weighted parameters are not allowed to be adjusted dynamically according to the current network status.
% which finally leads to the failure of guiding the optimization process on the right track. 
Generally, we believe that the policy learned by reward engineering might fall into the unexpected conditions. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/qoe2}
%     \caption{A QoE metric can evaluate several ABR algorithms, but the generated algorithm may deviate from the basic rules of the ABR if it blindly improves QoE score.}
%     \label{fig:qoe} 
% \end{figure}

\noindent \textbf{Summary.} In general, we observe that no matter how precisely and carefully the parameter of the linear-based reward function tunes, such tuned functions can hardly meet the requirement of any network conditions. E.g., the parameter of stable and unstable network conditions are not the same.
To that end, traditional learning-based scheme, which often optimizes the NN via the assigned functions, will eventually fail to provide a reliable performance on any network traces. We therefore, attempt to learn the strategies from the original demands. 

%Most prior research add additional smoothness metric $\left| r_k - r_{k-1} \right|$ to control the bitrate change of the entire session, while in practice the following metric is neglectable for the ABR algorithm~\cite{mao2019real}. Hence, in this work we also set the smoothness to zero for better understanding the fundamental performance of Zwei. We believe that Zwei can also solve $q_k$ with smoothness metric.

% \begin{itemize}
%     \item \textbf{\emph{How to train the NN without specific reward engineering?}}~As illustrated in Figure~\ref{fig:abr}, we use a simple ABR~(\S\ref{sec:background}) streaming example to illustrate the following observations. Recall that the goal of ABR algorithm is to select bitrates for the next chunk $k$ with high bitrate $r_k$ and less rebuffering time $t_k$, thus the optimization reward $q_k$ can be normally written as~\footnote{More details of QoE settings please refer to \color{darkgreen}{supplementary material}.}
%     \begin{equation}
%         q_k = r_k - \alpha t_k.
%     \end{equation}
%     Here $\alpha$ is the coefficient that adjust the importance of the underlying metrics. We evaluate the optimal strategy w.r.t the goal of ABR task on Figure~\ref{fig:abr2}. Experiment show that each network trace has its own \emph{optimal} reward function $q_k$ in different $\alpha$. The following results demystify an observation: recent learning-based studies leverage a reward function for optimizing the NN. However, they fail to perform well under the video transmission task since the real-world network condition is too variance that even influences the optimization objectives.
    
%     \textbf{Our Solution.} Motivated by the recent success of self-learning method~\cite{huang2018tiyuntsong},
    
%     \item \textbf{\emph{How to propose a learning algorithm which can use \emph{rule} or \emph{demand} to effectively update the NN?}}~Apparently, 
    
%     % \textbf{Our Solution.} Motivated by the recent success of self-learning method~\cite{huang2018tiyuntsong}, we adopt deep reinforcement learning (DRL) method to generalize strategies without any presumptions, aiming to adjust the buffer-bound to achieve high QoE performances dynamically. On the other hand, the buffer-bound method has better generalization, which helps NN effectively reduce the model size.
    
% \end{itemize}


==> Zwei 4/related.tex <==
\vspace{-10pt}
\section{Related Work}
\textbf{Heuristic Methods.}
\label{related:heu}
Heuristic-based ABR methods often adopts throughput prediction~(E.g., FESTIVE~\cite{jiang2014improving}) or buffer occupancy control~(E.g., BOLA~\cite{spiteri2016bola}) to handle the task.
However, such approaches suffer from either inaccurate bandwidth estimation or long-term bandwidth fluctuation problems.
Then, MPC~\cite{yin2015control} picks next chunks' bitrate by jointly considering throughput and buffer occupancy. Nevertheless, MPC is sensitive to its parameters since the it relies on well-understanding different network conditions. 
% What's more, Oboe~\cite{akhtar2018oboe} even proposes an auto-tuning method to tune the traditional heuristic methods to achieve better performance in different network settings.

Through preliminary measurements, it is widely accepted that the strategies are largely statically configured~\cite{adhikari2012unreeling}. In recent years, dynamic scheduling across different CSPs has received more attention. Jiang et. al.~\cite{jiang2017pytheas} uses E2 method to replace traditional model-based methods. 

\textbf{Learning-based Schemes.}
Recent years, several learning-based attempts have been made to tackle video transmission problem. For example, Mao et al.~\cite{mao2017neural} develop an ABR algorithm that uses DRL to select next chunks' bitrate.
% D-DASH~\cite{DDASH} uses Deep Q-learning method to perform a comprehensive evaluation based on state-of-the-art algorithms. 
Tiyuntsong optimizes itself towards a rule or a specific reward via the competition with two agents under the same network condition~\cite{huang2018tiyuntsong}. 
LTS~\cite{zhang2019enhancing} is a DRL-based scheduling approach which outperforms previously proposed CLS approaches. 
% Furthermore, QARC~\cite{QARC2018} optimizes a NN towards higher perceptual video quality and less stalling events. 
However, such methods fail to achieve actual requirements since they are optimized via a linear-based reward function.

==> ieee.tex <==
%\documentclass[10pt, letterpaper]{IEEEtran}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{comment}
\usepackage{color}
\usepackage{amsmath}
%\usepackage{subcaption}
\usepackage{booktabs} 
% For formal tables
\usepackage{multirow}
\usepackage{algorithm}
\usepackage{array}
\usepackage{enumitem}
\usepackage[noend]{algpseudocode}
\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}%
\PassOptionsToPackage{hyphens}{url}
%\usepackage{hyperref}
\usepackage[export]{adjustbox}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{colortbl}
\definecolor{mygray}{gray}{.9}
\usepackage{euscript}
\usepackage{amssymb}
\usepackage{algorithm,algpseudocode}
\usepackage{framed}
%\usetikzlibrary{automata, positioning, arrows, shapes}
\renewcommand{\arraystretch}{1.25}
\newcommand{\dtoprule}{\specialrule{1pt}{0pt}{0.4pt}%
\specialrule{0.3pt}{0pt}{\belowrulesep}%
}
\newcommand{\dbottomrule}{\specialrule{0.3pt}{0pt}{0.4pt}%
\specialrule{1pt}{0pt}{\belowrulesep}%
}

% colorful citation
 \usepackage{color}
 \usepackage{hyperref}
 \definecolor{darkred}{rgb}{0.6,0,0}
 \definecolor{darkgreen}{rgb}{0,0.5,0}
 \definecolor{darkblue}{rgb}{0,0.0,0.3}
 \hypersetup{colorlinks=true,
 		 %urlcolor=darkblue,
         linkcolor=darkred,
         citecolor=darkgreen
         }

\newcommand{\up}[1]{#1{}{\color{darkgreen}$\uparrow$}}
\newcommand{\down}[1]{#1{}{\color{darkred}$\downarrow$}}
         
% Compact itemize and enumerate.
\def\compactify{\itemsep=0pt \topsep=0pt \partopsep=0pt \parsep=0pt}
\let\latexusecounter=\usecounter
\newenvironment{CompactItemize}
  {\def\usecounter{\compactify\latexusecounter}
   \begin{itemize}\setlength{\leftmargin}{1.0em}}
  {\end{itemize}\let\usecounter=\latexusecounter}
\newenvironment{CompactEnumerate}
  {\def\usecounter{\setlength{\leftmargin}{1.75em}\compactify\latexusecounter}
   \begin{enumerate}}
  {\end{enumerate}\let\usecounter=\latexusecounter}        
%
% If IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it like:
% \documentclass[journal]{../sty/IEEEtran}





% Some very useful LaTeX packages include:
% (uncomment the ones you want to load)


% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.






% *** CITATION PACKAGES ***
%
%\usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.






% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex





% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath





% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.




% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig




% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix




%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
% endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% Axel Sommerfeldt. This package may be useful when used in conjunction with 
% IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% submissions have lists of figures/tables at the end of the paper and that
% figures/tables without any captions are placed on a page by themselves at
% the end of the document. If needed, the draftcls IEEEtran class option or
% \CLASSINPUTbaselinestretch interface can be used to increase the line
% spacing as well. Be sure and use the nomarkers option of endfloat to
% prevent endfloat from "marking" where the figures would have been placed
% in the text. The two hack lines of code above are a slight modification of
% that suggested by in the endfloat docs (section 8.4.1) to ensure that
% the full captions always appear in the list of figures/tables - even if
% the user used the short optional argument of \caption[]{}.
% IEEE papers do not typically make use of \caption[]'s optional argument,
% so this should not be an issue. A similar trick can be used to disable
% captions of packages such as subfig.sty that lack options to turn off
% the subcaptions:
% For subfig.sty:
% \let\MYorigsubfloat\subfloat
% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% However, the above trick will not work if both optional arguments of
% the \subfloat command are used. Furthermore, there needs to be a
% description of each subfigure *somewhere* and endfloat does not add
% subfigure captions to its list of figures. Thus, the best approach is to
% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% and instead reference/explain all the subfigures within the main caption.
% The latest version of endfloat.sty and its documentation can obtained at:
% http://www.ctan.org/pkg/endfloat
%
% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% later in the document, say, to conditionally put the References on a 
% page by themselves.




% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.




% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


\usepackage{dutchcal}
\begin{document}
%
% paper title
% Titles are generally capitalized except for words such as a, an, and, as,
% at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% not capitalized unless they are the first or last word of the title.
% Linebreaks \\ can be used within to get better formatting as desired.
% Do not put math or special symbols in the title.
\title{Learning Video Transmission Algorithms via Requirements}
%
% learning to generate strategies for various video transmission tasks via self-play reinforcement learning
% author names and IEEE memberships
% note positions of commas and nonbreaking spaces ( ~ ) LaTeX will not break
% a structure at a ~ so this keeps an author's name from being broken across
% two lines.
% use \thanks{} to gain access to the first footnote area
% a separate \thanks must be used for each paragraph as LaTeX2e's \thanks
% was not built to handle multiple paragraphs
%
\author{Tianchi Huang, Rui-Xiao Zhang, Lifeng Sun
% <-this % stops a space
\thanks{Corresponding Author: Lifeng Sun, mailto: sunlf@tsinghua.edu.cn.}%
\thanks{Media Lab, Tsinghua University.}
\thanks{Manuscript received July 21, 2019; revised Oct. 26, 2019.}
}

% note the % following the last \IEEEmembership and also \thanks - 
% these prevent an unwanted space from occurring between the last author name
% and the end of the author line. i.e., if you had this:
% 
% \author{....lastname \thanks{...} \thanks{...} }
%                     ^------------^------------^----Do not want these spaces!
%
% a space would be appended to the last name and could cause every name on that
% line to be shifted left slightly. This is one of those "LaTeX things". For
% instance, "\textbf{A} \textbf{B}" will typeset as "A B" not "AB". To get
% "AB" then you have to do: "\textbf{A}\textbf{B}"
% \thanks is no different in this regard, so shield the last } of each \thanks
% that ends a line with a % and do not let a space in before the next \thanks.
% Spaces after \IEEEmembership other than the last one are OK (and needed) as
% you are supposed to have spaces between the names. For what it is worth,
% this is a minor point as most people would not even notice if the said evil
% space somehow managed to creep in.



% The paper headers
%\markboth{Journal of \LaTeX\ Class Files,~Vol.~14, No.~8, August~2015}%
%{Shell \MakeLowercase{\textit{et al.}}: Bare Demo of IEEEtran.cls for IEEE Journals}
% The only time the second header will appear is for the odd numbered pages
% after the title page when using the twoside option.
% 
% *** Note that you probably will NOT want to include the author's ***
% *** name in the headers of peer review papers.                   ***
% You can use \ifCLASSOPTIONpeerreview for conditional compilation here if
% you desire.




% If you want to put a publisher's ID mark on the page you can do it like
% this:
%\IEEEpubid{0000--0000/00\$00.00~\copyright~2015 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.



% use for special paper notices
%\IEEEspecialpapernotice{(Invited Paper)}




% make the title area
\maketitle

% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\input{abs}
% Note that keywords are not normally used for peerreview papers.
\begin{IEEEkeywords}
Video transmission Strategy, Reinforcement Learning, Adaptive Bitrate Streaming.
\end{IEEEkeywords}






% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle

\input{intro}
\input{preliminaries}
\input{method}
\input{eval}
\input{related}
\input{conclusion}

% Can use something like this to put references on a page
% by themselves when using endfloat and the captionsoff option.
\ifCLASSOPTIONcaptionsoff
\newpage
\fi



% trigger a \newpage just before the given reference
% number - used to balance the columns on the last page
% adjust value as needed - may need to be readjusted if
% the document is modified later
%\IEEEtriggeratref{8}
% The "triggered" command can be changed if desired:
%\IEEEtriggercmd{\enlargethispage{-5in}}

% references section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
\bibliography{ref}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
% \begin{thebibliography}{1}
%\input{sample-sigconf.bbl}
% \begin{thebibliography}{1}

% \bibitem{IEEEhowto:kopka}
% H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
%   0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

% \end{thebibliography}

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
% \newpage
% \begin{IEEEbiography}{Tianchi Huang}
% received his M.E degree in the Department of Computer Science and Technology in Guizhou University in 2018. Currently he is a Ph.D student in the Department of Computer Science and Technology at Tsinghua University, advised by Prof. Lifeng Sun. 

% His research work focuses on the multimedia network streaming, including transmitting streams, overlay path construction and edge-assisted content delivery. He received Best Student Paper Awards presented by ACM Multimedia System 2019 Workshop.
% \end{IEEEbiography}

% \begin{IEEEbiography}{Rui-Xiao Zhang}
% received his B.E degree in Electronic Engineering Department in Tsinghua University in 2017. Currently, he is pursuing his Ph.D candidate in Department of Computer Science and Technology, Tsinghua University, China. 

% His research interests lie in the area of content delivery networks, the optimization of multimedia streaming and cloud computing. He received Best Student Paper Awards presented by ACM Multimedia System 2019 Workshop.
% \end{IEEEbiography}

% \begin{IEEEbiography}{Lifeng Sun}
% received the B.S and Ph.D degrees in system engineering from National University of Defense Technology, Changsha, Hunan, China, in 1995 and 2000, respectively. He joined Tsinghua University since 2001.
% He is currently a Professor with the Computer Science and Technology Department of Tsinghua University, Beijing.

% Dr.Sun's research interests include the area of networked multimedia, video streaming, 3D/multiview video coding, multimedia cloud computing, and social media.
% \end{IEEEbiography}

% if you will not have a photo at all:

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks
\end{document}



